Data-driven Nonlinear Predictive Control for Feedback Linearizable Systems

We present a data-driven nonlinear predictive control approach for the class of discrete-time multi-input multi-output feedback linearizable nonlinear systems. The scheme uses a non-parametric predictive model based only on input and noisy output data along with a set of basis functions that approximate the unknown nonlinearities. Despite the noisy output data as well as the mismatch caused by the use of basis functions, we show that the proposed multistep robust data-driven nonlinear predictive control scheme is recursively feasible and renders the closed-loop system practically exponentially stable. We illustrate our results on a model of a fully-actuated double inverted pendulum.

==> sections/App.tex <==
\appendix
\subsection{The block-Brunovsky canonical form}\label{Bruno_app}
	The matrices $\left(\mathcal{A,B,C}\right)$ have the following form\cite{Zeitz89}
	\begin{equation*}
		\begin{matrix}
			\mathcal{A} \hspace{-0.5mm}\coloneqq\hspace{-1mm} \begin{bmatrix}
			A_1 \hspace{-1mm} & \hspace{-1mm} \dots \hspace{-1mm} & \hspace{-1mm} \mathbf{0}\\
			\vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm}&\hspace{-1mm} \vdots\\
			\mathbf{0} \hspace{-1mm}& \hspace{-1mm}\dots\hspace{-1mm} & \hspace{-1mm}A_{m}
			\end{bmatrix}\hspace{-1mm},\hspace{-1mm} &\hspace{-1mm} \mathcal{B} \hspace{-0.5mm}\coloneqq \hspace{-1mm}\begin{bmatrix}
			B_1 \hspace{-1mm} & \hspace{-1mm} \dots \hspace{-1mm} & \hspace{-1mm} \mathbf{0}\\
			\vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm}&\hspace{-1mm} \vdots\\
			\mathbf{0} \hspace{-1mm}& \hspace{-1mm}\dots\hspace{-1mm} & \hspace{-1mm}B_{m}
		\end{bmatrix}\hspace{-1mm},\hspace{-1mm}&\hspace{-1mm}\mathcal{C} \hspace{-0.5mm}\coloneqq\hspace{-1mm} \begin{bmatrix}
				C_1 \hspace{-1mm} & \hspace{-1mm} \dots \hspace{-1mm} & \hspace{-1mm} \mathbf{0}\\
				\vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm}&\hspace{-1mm} \vdots\\
				\mathbf{0} \hspace{-1mm}& \hspace{-1mm}\dots\hspace{-1mm} & \hspace{-1mm}C_{m}
			\end{bmatrix}
		\end{matrix}\hspace{-0.5mm},
%		\begin{aligned}
%			&\begin{matrix}
%				\mathcal{A} \coloneqq \begin{bmatrix}
%					A_1 & \dots & 0\\
%					\vdots & \ddots & \vdots\\
%					0 & \dots & A_{m}
%				\end{bmatrix}, & \mathcal{B}\coloneqq \begin{bmatrix}
%					B_1 & \dots& 0\\
%					\vdots & \ddots & \vdots\\
%					0 & \dots & B_{m}
%				\end{bmatrix}
%			\end{matrix}\\
%			&\,\mathcal{C} \coloneqq \begin{bmatrix}
%				C_1 & \dots& 0\\
%				\vdots & \ddots & \vdots\\
%				0 & \dots & C_{m}
%			\end{bmatrix}
%		\end{aligned}
	\end{equation*}
	with each $A_i,B_i,C_i$ for $i\in\mathbb{Z}_{[1,m]}$ defined as the following controllable and observable triplet
	\begin{equation*}
		\begin{aligned}
			&\begin{matrix}
				A_i \coloneqq \begin{bmatrix}
					0&1&\dots&0 \\ \vdots&\ddots&\ddots&\vdots \\ \vdots& &\ddots&1 \\ 0&\dots&\dots&0
				\end{bmatrix}, &
				B_i \coloneqq \begin{bmatrix}
					0\\ \vdots\\ 0\\ 1
				\end{bmatrix}, &C_i^\top \coloneqq \begin{bmatrix}
				1 \\ 0 \\ \vdots \\ 0
			\end{bmatrix}
			\end{matrix}
		\end{aligned}
	\end{equation*}
	%%%%%%%%%%%%%
	\subsection{Proof of Lemma \ref{lemma_controllable_pair}}\label{app_controllable_pair}
	A necessary and sufficient condition for controllability of $(\mathcal{A,BG})$ is that the following matrix has full row rank
	\begin{equation}
		\begin{aligned}
			&\begin{bmatrix}\mathcal{BG} & \mathcal{ABG}  & \dots & \mathcal{A}^{n-1}\mathcal{BG} \end{bmatrix}\\
			&= \begin{bmatrix}
				B_1g_1^\top & A_1B_1g_1^\top & \cdots & A_1^{n-1}B_1g_1^\top\\
				\vdots & \vdots & \ddots & \vdots\\
				B_mg_m^\top & A_mB_mg_m^\top & \cdots & A_m^{n-1}B_mg_m^\top
			\end{bmatrix}.\label{ctrb_ABG_step1}
		\end{aligned}
	\end{equation}
	\indent By the structure of $(A_i,B_i)$ in Appendix \ref{Bruno_app}, each block row of \eqref{ctrb_ABG_step1} has the following form
	\begin{equation}
		\begin{aligned}
			&\begin{bmatrix}
				B_ig_i^\top & A_iB_ig_i^\top & \cdots & A_i^{n-1}B_ig_i^\top
			\end{bmatrix}\\[3ex]
			&=\left[
			\begin{array}{ccccc}
				\mathbf{0}& \cdots & \mathbf{0}& g_i^\top & \bovermat{$(\hspace{-0.25mm}n\hspace{-0.5mm}-\hspace{-0.5mm}d_i\hspace{-0.25mm})r\hspace{-0.25mm}$ cols}{\mathbf{0}\quad \cdots \quad\mathbf{0}} \\
				\mathbf{0}& \cdots & g_i^\top & \mathbf{0}& \mathbf{0}\quad \cdots \quad \mathbf{0}\\
				\vdots & \scalebox{-1}[1]{$\ddots$} & \vdots & \vdots & \vdots \quad \cdots \quad \vdots \\
				g_i^\top & \cdots & \mathbf{0}& \mathbf{0}& \mathbf{0}\quad \cdots \quad \mathbf{0}\\
			\end{array}
			\right],
		\end{aligned}\label{ctrb_ABG_step2}
	\end{equation}
	which clearly has full row rank (i.e., rank $=d_i$) since $\mathcal{G}$ is full row rank and, hence, no row $g_i^\top$ is all zeros. Since, again, $\mathcal{G}$ is full row rank, then the concatenation of the block rows of the form in \eqref{ctrb_ABG_step2} results in a full row rank matrix \eqref{ctrb_ABG_step1} (i.e., rank $=\sum_id_i=n$), implying that the pair $(\mathcal{A,BG})$ is controllable.
%	Note that the pair $(\mathcal{A,B})$ is controllable by definition of the block-Brunovsky canonical form and hence 
%	\begin{equation*}
%		\begin{aligned}
%			&\begin{bmatrix}\mathcal{B} & \mathcal{AB}  & \dots & \mathcal{A}^{n-1}\mathcal{B} \end{bmatrix}\\
%			& = \hspace{-1mm} \begin{bmatrix}
%				B_1 \hspace{-1mm} & \hspace{-1mm} \cdots \hspace{-1mm} & \hspace{-1mm} \mathbf{0} \hspace{-1mm} & \hspace{-1mm} A_1B_1 \hspace{-1mm} & \hspace{-1mm} \cdots \hspace{-1mm} & \hspace{-1mm} \mathbf{0} \hspace{-1mm} & \hspace{-1mm} A_1^{n-1}B_1  \hspace{-1mm} & \hspace{-1mm} \cdots \hspace{-1mm} & \hspace{-1mm} \mathbf{0}\\
%				\vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm} & \hspace{-1mm} \vdots \hspace{-1mm} & \hspace{-1mm} \vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm} & \hspace{-1mm} \vdots \hspace{-1mm} & \hspace{-1mm} \vdots \hspace{-1mm} & \hspace{-1mm} \ddots \hspace{-1mm} & \hspace{-1mm} \vdots\\
%				\mathbf{0} \hspace{-1mm} & \hspace{-1mm}  \cdots \hspace{-1mm} & \hspace{-1mm} B_m \hspace{-1mm} & \hspace{-1mm} \mathbf{0} \hspace{-1mm} & \hspace{-1mm} \cdots \hspace{-1mm} & \hspace{-1mm} A_mB_m \hspace{-1mm} & \hspace{-1mm} \mathbf{0} \hspace{-1mm} & \hspace{-1mm} \cdots \hspace{-1mm} & \hspace{-1mm} A_m^{n-1}B_m
%			\end{bmatrix}
%		\end{aligned}
%	\end{equation*}
%	has full row rank. From here, it can be seen that each block row of the following matrix
%	\begin{equation*}
%		\begin{aligned}
%			&\begin{bmatrix}\mathcal{B} & \mathcal{AB}  & \dots & \mathcal{A}^{n-1}\mathcal{B} \end{bmatrix}(I\otimes \mathcal{G})\\
%			&= \begin{bmatrix}
%				B_1g_1^\top & A_1B_1g_1^\top & \cdots & A_1^{n-1}B_1g_1^\top\\
%				\vdots & \vdots & \ddots & \vdots\\
%				B_mg_m^\top & A_mB_mg_m^\top & \cdots & A_m^{n-1}B_mg_m^\top
%			\end{bmatrix}
%		\end{aligned}
%	\end{equation*}
%%	\begin{multline*}
%%		\begin{aligned}
%%			&\begin{bmatrix}\mathcal{B} & \mathcal{AB}  & \dots & \mathcal{A}^{n-1}\mathcal{B} \end{bmatrix}(I\otimes \mathcal{G})\\
%%			&\quad=
%%			\left[
%%			\begin{matrix}
%%				B_1g_1^\top  &  \cdots  &  \mathbf{0}  &  A_1B_1g_1^\top  &  \cdots  &  \mathbf{0}\\
%%				\vdots  &  \ddots  &  \vdots  &  \vdots  &  \ddots  &  \vdots\\
%%				\mathbf{0}  &   \cdots  &  B_mg_m^\top  &  \mathbf{0}  &  \cdots  &  A_mB_mg_m^\top
%%			\end{matrix}
%%			\right.
%%			\\
%%			&\hspace{3.5cm}\left.
%%			\begin{matrix}
%%				A_1^{n-1}B_1g_1^\top   &  \cdots  &  \mathbf{0}\\
%%				\vdots  &  \ddots  &  \vdots\\
%%				\mathbf{0}  &  \cdots  &  A_m^{n-1}B_mg_m^\top
%%			\end{matrix}
%%			\right]
%%		\end{aligned}
%%	\end{multline*}
%	also has full row rank. This is because each $(A_i,B_i)$ is a controllable pair and $\mathcal{G}$ is full row rank by Assumption \ref{rank_assmp_G} (and hence no row of $\mathcal{G}$ (i.e., $g_i^\top$) is all zeros). Therefore, the matrix $\begin{bmatrix}\mathcal{B}\mathcal{G} & \mathcal{AB}\mathcal{G} & \dots & \mathcal{A}^{n-1}\mathcal{B}\mathcal{G}\end{bmatrix}$ has full row rank which in turn implies that $(\mathcal{A,BG})$ is a controllable pair.\qed
%\subsection{Proof of Lemma \ref{lemma_eps_zero}}
%\label{lemma_proof_app}
%	From \eqref{err_sim}, it can be seen that the error bound would go to zero as $\varepsilon^*\to 0$, \emph{if} \textbf{(i)} $\norm*{\alpha^*}$ remains bounded and \textbf{(ii)} $c^\top c\to0$. To show these two properties, we start by proposing the following candidate solution for the optimization problem in \eqref{alpha*}
%	\begin{equation}
%		\bar{\alpha} = \hspace{-1mm}\begin{bmatrix}
%			H_{L}(\hat{\Psi}(\mathbf{u,y})+\hat{E}(\mathbf{u,y}))\\
%			H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ H_{d_m}(y_{m,[0,N-L+d_m-1]})
%		\end{bmatrix}^\dagger\hspace{-1mm}\begin{bmatrix}
%			\hat{\Psi}(\mathbf{\bar{u}},\mathbf{\bar{y}}) + \hat{E}(\mathbf{\bar{u}},\mathbf{\bar{y}})\\
%			\bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}
%		\end{bmatrix}.
%	\end{equation}
%	Since $\hat{\Psi}(\mathbf{u,y})+\hat{E}(\mathbf{u,y})$ is persistently exciting of order $L+n$, then by Theorem \ref{MIMO_sim_thm}, the above choice $\bar{\alpha}$ is well defined. By optimality, we have that $J(\alpha^*)\leq J(\bar{\alpha})$, or
%	\begin{equation*}
%		\begin{aligned}
%			&\overbrace{\norm*{\hspace{-0.5mm}\begin{bmatrix}
%						H_{L}(\hat{\Psi}(\mathbf{u},\mathbf{y}))\\ H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ \hspace{-0.5mm}H_{d_m}(y_{m,[0,N-L+d_m-1]})
%					\end{bmatrix}\hspace{-1mm}\alpha^* \hspace{-01mm}-\hspace{-1mm} \begin{bmatrix}
%						\hat{\Psi}(\mathbf{\bar{u}},\mathbf{\hat{y}})\\ \bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}
%					\end{bmatrix}\hspace{-0.5mm}}_2^2}^{=c^\top c}\hspace{-2mm}+ \hspace{0mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\\
%			&\hspace{-1mm}\leq\hspace{-1mm}\norm*{\hspace{-0.5mm}\begin{bmatrix}
%					H_{L}(\hat{\Psi}(\mathbf{u},\mathbf{y}))\\ H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ \hspace{-0.5mm}H_{d_m}(y_{m,[0,N-L+d_m-1]})
%				\end{bmatrix}\hspace{-1mm}\bar{\alpha}\hspace{-1mm}-\hspace{-1mm}\begin{bmatrix}
%					\hat{\Psi}(\mathbf{\bar{u}},\mathbf{\bar{y}})\\ \bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}
%				\end{bmatrix}\hspace{-0.5mm}}_2^2\hspace{-2mm}+\hspace{-1mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.
%		\end{aligned}
%	\end{equation*}
%	Using \eqref{subset_of_unsolvable}, this can be rewritten as\footnote{Here, $\mathbf{0}$ denotes a block of zeros of appropriate dimensions}
%	\begin{align}
%		&\norm*{\hspace{-0.5mm}\begin{bmatrix}
%				\hat{E}(\mathbf{\bar{u}},\mathbf{\hat{y}}) \\ \boldsymbol{0}
%			\end{bmatrix}\hspace{-1mm}-\hspace{-1mm} \begin{bmatrix}
%				H_{L-d_q}(\hat{E}(\mathbf{u,y})) \\ \boldsymbol{0}
%			\end{bmatrix}\hspace{-1mm}\alpha^*\hspace{-0.25mm}}_2^2\hspace{-1mm}+ \hspace{-0.5mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\label{RHS_to_0}\\
%		&\hspace{0mm}\leq\hspace{0mm}\norm*{\hspace{-0.5mm}\begin{bmatrix}
%				\hat{E}(\mathbf{\bar{u}},\mathbf{\bar{y}}) \\ \boldsymbol{0}
%			\end{bmatrix}\hspace{-1mm}-\hspace{-1mm}\begin{bmatrix}
%				H_{L-d_q}(\hat{E}(\mathbf{u,y})) \\ \boldsymbol{0}
%			\end{bmatrix}\hspace{-0.5mm}\bar{\alpha}}_2^2\hspace{-1mm}+\hspace{-0.5mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.\notag
%	\end{align}
%	\indent It is clear from \eqref{RHS_to_0} that the right hand side of the inequality goes to zero as $\hat{E}(\cdot,\cdot)\to0$ \emph{as long as $\norm*{\bar{\alpha}}$ is bounded}\footnote{From \eqref{tilde_E_bdd_asmp}, it can be seen that $\hat{E}(\cdot,\cdot)$ goes to zero as $\varepsilon^*\to0$.}. This in turn implies that the left hand side, which is a sum of two non-negative terms, goes to zero as well, implying \textbf{(ii)}. Now, it is only left to be shown that $\norm*{\bar{\alpha}}$ is bounded.\par
%	Notice from \eqref{basis}, that $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ can be viewed as a measure of how much does the linear combination of basis functions $\mathcal{G}\hat{\Psi}(\mathbf{u,y})$ differ from the linear combination of \emph{a correct} choice of basis functions $\mathcal{W}\hspace{-2mm}\stackrel{*}{\Psi}\hspace{-2mm}(\mathbf{u,y})$ such that $\Phi(\mathbf{u}_k,\Xi_k) = \sum\limits_{i=1}^{s}\mu_i\stackrel{*}{\psi}_{i}\hspace{-1mm}(\mathbf{u}_k,\Xi_k)$, for $\mu_i\geq0$. Specifically,
%	\begin{equation*}
%		\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k) = \mathcal{W}\hspace{-0.75mm}\stackrel{*}{\Psi}_k\hspace{-1mm}(\mathbf{u,y}) - \mathcal{G}\hat{\Psi}_k(\mathbf{u,y}).
%	\end{equation*}
%	Recall again that $\bar{\alpha}$ is one such that
%	\begin{equation*}
%		\begin{bmatrix}
%			H_{L}(\hat{\Psi}(\mathbf{u,y})+\hat{E}(\mathbf{u,y}))\\
%			H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ H_{d_m}(y_{m,[0,N-L+d_m-1]})
%		\end{bmatrix} \hspace{-1mm}\bar{\alpha} =\hspace{-1mm}\begin{bmatrix}
%			\hat{\Psi}(\mathbf{\bar{u}},\mathbf{\bar{y}}) + \hat{E}(\mathbf{\bar{u}},\mathbf{\bar{y}})\\
%			\bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}
%		\end{bmatrix},
%	\end{equation*}
%	which can be rewritten as
%	\begin{equation*}
%		\begin{bmatrix}
%			H_{L}(\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{u,y})+\Delta\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{u,y}))\\
%			H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ H_{d_m}(y_{m,[0,N-L+d_m-1]})
%		\end{bmatrix} \hspace{-1mm}\bar{\alpha} =\hspace{-1mm}\begin{bmatrix}
%			\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{\bar{u}},\mathbf{\bar{y}}) +\Delta\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{\bar{u}},\mathbf{\bar{y}})\\
%			\bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}
%		\end{bmatrix},
%	\end{equation*}
%	with $\Delta\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\cdot,\cdot)=\hat{\Psi}(\cdot,\cdot)+\hat{E}(\cdot,\cdot)-\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\cdot,\cdot)$. Next, we rearrange the terms and define the following matrices
%	\begin{align}
%		&\left(\overbrace{\begin{bmatrix}H_{L}(\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{u,y}))\\ H_{d_1}(y_{1,[0,N-L+d_1-1]}) \\ \vdots \\ H_{d_m}(y_{m,[0,N-L+d_m-1]})\end{bmatrix}}^{\eqqcolon A} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}H_{L}(\Delta\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{u,y}))\\ \boldsymbol{0}\\\vdots\\\boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta A}\right) \bar{\alpha}\notag\\
%		&=\left(\overbrace{\begin{bmatrix}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{\bar{u}},\mathbf{\bar{y}}) \\ \bar{y}_{1,[0,d_1-1]} \\ \vdots \\ \bar{y}_{m,[0,d_m-1]}\end{bmatrix}}^{\eqqcolon b} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{\bar{u}},\mathbf{\bar{y}}) \\ \boldsymbol{0}\\\vdots\\\boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta b}\right).\label{Golub}
%	\end{align}
%	\indent Notice that for a \emph{fixed} $\mathbf{\bar{u}},\mathbf{\bar{y}}$, \eqref{Golub} represents a perturbed under-determined system of linear equations. Therefore, by applying results from perturbation theory of under-determined system \cite[Theorem 5.6.1]{Golub12}, it can be shown that
%	\begin{equation}
%		\frac{\norm*{\bar{\alpha}-\alpha_{\textup{bnd}}}_2}{\norm*{\alpha_{\textup{bnd}}}_2}\leq\kappa_2(A)\left(c_0\frac{\norm*{\Delta A}_2}{\norm*{A}_2} + \frac{\norm*{\Delta b}_2}{\norm*{b}_2}\right) + O(\sigma^2),\label{pertb_lin_sys}
%	\end{equation}
%	where $\alpha_{\textup{bnd}}=A^\dagger b$ is the \textit{bounded} minimum-norm solution of the unperturbed system of equations and $\kappa_2(A)=\norm*{A}_2\norm*{A^\dagger}_2$ is the condition number of the matrix $A$. Moreover,\footnote{$n_{c,A},\,n_{r,A}$ are the numbers of columns and rows of matrix $A$, respectively.} $c_0\coloneqq\min{\left\lbrace2, n_{c,A}-n_{r,A}+1\right\rbrace}$ and $\sigma\coloneqq\max{\left\lbrace\frac{\norm*{\Delta A}_2}{\norm*{A}_2},\frac{\norm*{\Delta b}_2}{\norm*{b}_2}\right\rbrace}$.\par
%	From \eqref{pertb_lin_sys}, it can be seen that as $\varepsilon^*\to0$, the term $\Delta\hspace{-1mm}\stackrel{*}{\Psi}\hspace{-1mm}(\mathbf{u,y})\to0$ and the candidate $\bar{\alpha}$ approaches the bounded solution $\alpha_{\textup{bnd}}$. Therefore, the RHS of \eqref{RHS_to_0} approaches zero as $\varepsilon^*\to 0$ and consequently, the LHS as well, which completes the proof.\qed
\subsection{Proof of Theorem \ref{MIMO_inexact_om_thm}}\label{proof_om_app}
By definition of $\alpha^*$ from \eqref{alpha*2} and for some $c$ in the theorem statement, it holds that
\begin{equation}
	\begin{bmatrix}
		H_{L}(\hat{\Psi}(\mathbf{u},\Xi))\\ H_{L+1}(\Xi)
	\end{bmatrix}\alpha^* = \begin{bmatrix}
		\hat{\Psi}(\overbrace{H_{L}(\mathbf{u})\alpha^*}^{\hat{\mathbf{u}}\coloneqq},\bar{\Xi})\\ \bar{\Xi}
	\end{bmatrix} + \overbrace{\begin{bmatrix}
			c_{\Psi}\\ c_{\Xi}
	\end{bmatrix}}^{\coloneqq c}\hspace{-1mm}.
	\label{sim_om}
\end{equation}
The constraint in \eqref{alpha*2_b} fixes $\hat{\Xi}_0 = H_1(\Xi_{[0,N-L]})\alpha = \bar{\Xi}_0$ and hence $e_{i,[0,d_i-1]}=\bar{y}_{i,[0,d_i-1]}-\hat{y}_{i,[0,d_i-1]} = \mathbf{0}$.\par 
We denote the corresponding element of $c_{\Xi,j}$ in \eqref{sim_om} to each output instant $\bar{y}_{i,j}$ as $c_{y_{i,j}}$, for all $i\in\mathbb{Z}_{[1,m]}$ and all $j\in\mathbb{Z}_{[0,L+d_i-1]}$. Furthermore, it can be seen from the second block row of \eqref{sim_om} that every instance of each reference trajectory $\bar{y}_{i}$ can be written as %, for all $i\in\mathbb{Z}_{[1,m]}$ and all $k\in\mathbb{Z}_{[d_i,L+d_i-2]}$,
\begin{align}
	\bar{y}_{i,k+d_i} &=H_1({y}_{i,[k+d_i,k+d_i+N-L]})\alpha^*-c_{{y}_{i,k+d_i}}\notag
	\\&\stackrel{\eqref{y_for_proofs}}{=}g_i^\top H_1(\hat{\Psi}_{[k,k+N-L]}(\mathbf{u},\Xi))\alpha^*\notag
	\\&\quad+H_1(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi))\alpha^*-c_{{y}_{i,k+d_i}}\notag
	%
	\\&\stackrel{\eqref{sim_om}}{=}g_i^\top\left(\hat{\Psi}_{k}(\hat{\mathbf{u}},\bar{\Xi}) + c_{\Psi,k}\right)\label{e_vector_om}
	\\&\quad+ H_1(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi))\alpha^*-c_{{y}_{i,k+d_i}}\notag
	%
	\\&\stackrel{\eqref{basis}}{=}\phi_i(\hat{\mathbf{u}}_{k},\bar{\Xi}_{k})-{\varepsilon}_i(\hat{\mathbf{u}}_{k},\bar{\Xi}_{k})+ g_i^\top c_{\Psi,k} \notag
	\\&\quad+  H_1(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi))\alpha^*-c_{{y}_{i,k+d_i}},\notag
\end{align}
%It can be seen here that the only difference between \eqref{e_vector_om} and \eqref{sim_e_vector} is the appearance of an additional entry of the $c$ vector in \eqref{e_vector_om}.
for $k\in\mathbb{Z}_{[0,L-1]}$. Next, by applying $\hat{\mathbf{u}}=H_L(\mathbf{u})\alpha^*$ to the nonlinear system \eqref{Lsys3}, we obtain $\hat{y}_{i,k+d_i} \stackrel{\eqref{y_for_proofs}}{=} \phi_i(\hat{\mathbf{u}}_k,\hat{\Xi}_k)$. Therefore, the error between the reference output trajectory and the approximate one is given by
\begin{equation}
	\begin{aligned}
		e_{i,k+d_i} &= \bar{y}_{i,k+d_i} - \hat{y}_{i,k+d_i}\\
		&=\phi_i(\hat{\mathbf{u}}_{k},\bar{\Xi}_{k})-{\varepsilon}_i(\hat{\mathbf{u}}_{k},\bar{\Xi}_{k})+ g_i^\top c_{\Psi,k}\\
		&\quad+  H_1(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi))\alpha^*-c_{{y}_{i,k+d_i}}\\
		&\quad-\phi_i(\hat{\mathbf{u}}_k,\hat{\Xi}_k),
	\end{aligned}\label{bounding_om_terms}
\end{equation}
for $k\in\mathbb{Z}_{[0,L-1]}$. From this point, the remainder of the proof follows analogous steps as the proof of Theorem \ref{MIMO_inexact_sim_thm} from \eqref{sim_e_vector} on.
\qed
%%%%%%%%%%%%%%%
%\subsection{Vanishing output matching error for vanishing basis functions approximation error}\label{lemma_eps_zero_OM}
%This result is the dual result to Lemma \ref{lemma_eps_zero}. 
%\begin{lemma}
%	Suppose that the conditions of Theorem \ref{MIMO_inexact_om_thm} hold and let $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ be persistently exciting of order $L+n$.
%	Then, as $\varepsilon^*\to0$, the error $e_{i,[0,L+d_i-1]}\to0$ as well.
%\end{lemma}
%\begin{proof}
%	It can be seen from \eqref{err_om} that, for each fixed $k$, the error bound goes to zero as $\varepsilon^*\to 0$ \emph{if} \textbf{(i)} $\norm*{\alpha^*}_1$ is bounded and \textbf{(ii)} $c^\top c\to0$ as $\varepsilon^*\to 0$. To show these two properties, we start by proposing a candidate solution for the optimization problem in \eqref{alpha*2}. For sufficiently small $\varepsilon^*$, persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ implies that of $\{\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ of the same order. Therefore, using \eqref{subset_of_unsolvable}, we make the following choice of $\bar{\alpha}$
%	\begin{equation}
%		\hspace{-3mm}\bar{\alpha} = \hspace{-1mm}\begin{bmatrix}\hspace{-0.5mm}
%			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}^{\dagger}\begin{bmatrix}
%			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}_0
%		\end{bmatrix}\hspace{-1mm}.\label{alpha_bar_definition2}
%	\end{equation}
%	This holds since, given the assumed persistency of excitation condition, the pseudoinverse in \eqref{alpha_bar_definition2} is in fact a right inverse of the matrix on the left hand side of \eqref{subset_of_unsolvable} (cf. \cite{Willems05}). Moreover, by Theorem \ref{DB_MIMO_rep}, this choice of $\bar{\alpha}$ satisfies the following equation
%	\begin{equation}
%		\begin{bmatrix}\hspace{-0.5mm}
%			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{L+1}(\Xi)\end{bmatrix}\bar{\alpha} = \hspace{-1mm}\begin{bmatrix}
%			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ \bar{\Xi}
%		\end{bmatrix}\hspace{-1mm},\label{alphabar_satisfies_OM}
%	\end{equation}
%	and, hence, is a candidate solution for \eqref{alpha*2}. By optimality, we have that $J(\alpha^*)\leq J(\bar{\alpha})$, or
%	\begin{equation*}
%		\begin{aligned}
%			&\overbrace{\norm*{\hspace{-0.5mm}\begin{bmatrix}
%						H_L(\hat{\Psi}(\mathbf{u},\Xi)) \\ H_{L+1}(\Xi)
%					\end{bmatrix}\alpha^* - \begin{bmatrix}
%						\hat{\Psi}(H_L(\mathbf{u})\alpha^*,\bar{\Xi}) \\ \bar{\Xi}\end{bmatrix}\hspace{-0.5mm}}_2^2}^{\stackrel{\eqref{sim_om}}{=}c^\top c}\hspace{-2mm}+ \hspace{0mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\\
%			&\hspace{-1mm}\leq\hspace{-1mm}\norm*{\hspace{-0.5mm}\begin{bmatrix}
%					H_L(\hat{\Psi}(\mathbf{u},\Xi)) \\ H_{L+1}(\Xi)
%				\end{bmatrix}\bar{\alpha} - \begin{bmatrix}
%					\hat{\Psi}(H_L(\mathbf{u})\bar{\alpha},\bar{\Xi}) \\ \bar{\Xi}\end{bmatrix}\hspace{-0.5mm}}_2^2\hspace{-2mm}+\hspace{-1mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.
%		\end{aligned}
%	\end{equation*}
%	{Using} \eqref{alphabar_satisfies_OM}, this can be rewritten as
%	\begin{equation}
%		c^\top c+ \hspace{-0.5mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\hspace{0.1mm}\leq\hspace{0.1mm}\norm*{\hspace{-0.5mm}
%			\hat{E}(\mathbf{\bar{u}},\bar{\Xi})
%			\hspace{-1mm}-\hspace{-1mm}
%			H_{L}(\hat{E}(\mathbf{u},\Xi))
%			\hspace{-0.15mm}\bar{\alpha}}_2^2\hspace{-1mm}+\hspace{-0.5mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.\label{RHS_to_02}
%	\end{equation}
%	\indent It is clear that the right hand side of \eqref{RHS_to_02} goes to zero as $\hat{E}(\mathbf{u},\Xi)\to0$ (cf. \eqref{tilde_E_bdd_asmp}) {as long as $\norm*{\bar{\alpha}}_2$ is bounded}. As a result, the left hand side, which is a sum of two non-negative terms, goes to zero as well, implying point \textbf{(ii)} above. Hence, it is only left to show that $\norm*{\bar{\alpha}}_2$ is bounded.\par
%	Recall from \eqref{alpha_bar_definition2} that $\bar{\alpha}$ satisfies the following
%	\begin{equation*}
%		\hspace{-1mm}\begin{bmatrix}\hspace{-0.5mm}
%			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}\bar{\alpha} = \begin{bmatrix}
%			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}_0
%		\end{bmatrix},
%	\end{equation*}
%	which can be rewritten as
%	\begin{gather}
%		\hspace{-20mm}\left(\overbrace{\begin{bmatrix}H_{L}(\hat{\Psi}(\mathbf{u},\Xi))\\ H_{1}(\Xi_{[0,N-L]})\end{bmatrix}}^{\eqqcolon \Theta} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}H_{L}(\hat{E}(\mathbf{u},\Xi))\\ \boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta \Theta}\right) \bar{\alpha}\notag\\
%		\hspace{15mm}=\left(\overbrace{\begin{bmatrix}\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi})\\ \bar{\Xi}_0 \end{bmatrix}}^{\eqqcolon \mu} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}\hat{E}(\mathbf{\bar{u}},\bar{\Xi}) \\ \boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta \mu}\right).\label{Golub2}
%	\end{gather}
%	\indent Notice that for a \emph{fixed} matched trajectory $\mathbf{\bar{u}},\bar{\Xi}$, \eqref{Golub2} represents a perturbed under-determined system of linear equations. Therefore, by applying results from perturbation theory of under-determined system \cite[Theorem 5.6.1]{Golub12}, it can be shown that
%	\begin{equation}
%		\frac{\norm*{\bar{\alpha}-\alpha_{\textup{bnd}}}_2}{\norm*{\alpha_{\textup{bnd}}}_2}\leq\kappa_2(\Theta)\left(c_0\frac{\norm*{\Delta \Theta}_2}{\norm*{\Theta}_2} + \frac{\norm*{\Delta \mu}_2}{\norm*{\mu}_2}\right) + O(\sigma^2),\label{pertb_lin_sys2}
%	\end{equation}
%	where $\alpha_{\textup{bnd}}=\Theta^\dagger \mu$ is the \textit{bounded} minimum-norm solution of the unperturbed system of equations and $\kappa_2(\Theta)=\norm*{\Theta}_2\norm*{\Theta^\dagger}_2$ is the condition number of the matrix $\Theta$. Moreover, $c_0\coloneqq\min{\left\lbrace2, n_{c,\Theta}-n_{r,\Theta}+1\right\rbrace}$ and $\sigma\coloneqq\max{\left\lbrace\frac{\norm*{\Delta \Theta}_2}{\norm*{\Theta}_2},\frac{\norm*{\Delta \mu}_2}{\norm*{\mu}_2}\right\rbrace}$.\par
%	From \eqref{Golub2}, it can be seen that as $\varepsilon^*\to0$, the terms $\Delta\Theta,\,\Delta\mu\to0$ and, by \eqref{pertb_lin_sys2}, the candidate $\bar{\alpha}$ approaches the bounded solution $\alpha_{\textup{bnd}}$, which is finite for any fixed $\mathbf{\bar{u}},\bar{\Xi}$. Therefore, the right hand side of \eqref{RHS_to_02} approaches zero as $\varepsilon^*\to 0$ and consequently, the left hand side does as well, which completes the proof.
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fully actuated double inverted pendulum parameters}
\label{robot_params_app}
The matrices $M(\theta), C(\theta,\dot{\theta})$, the vector $g(\theta)$ and their elements are given by
\begin{align*}
	&\begin{matrix}
		M(\theta) \hspace{-1mm}\coloneqq \hspace{-1mm}\begin{bmatrix}
			M_{11} & M_{12} \\ M_{21} & M_{22}
		\end{bmatrix}\hspace{-1mm},\hspace{-1mm}
		&\hspace{-1mm}
		C(\theta,\dot{\theta}) \hspace{-1mm}\coloneqq\hspace{-1mm} \begin{bmatrix}
			C_{11} & C_{12} \\ C_{21} & C_{22}
		\end{bmatrix}\hspace{-1mm},\hspace{-1mm}
		&\hspace{-1mm}
		g(\theta)\hspace{-1mm} \coloneqq \hspace{-1mm}\begin{bmatrix}
			g_{11} \\ g_{21}
		\end{bmatrix}\hspace{-0.5mm}
	\end{matrix},\notag\\
	&M_{11} = m_1l_{c1}^2+I_1+m_2(l_{1}^2 + l_{c2}^2 + 2l_1l_{c2}\cos(\theta_2(t)))+I_2,\notag\\
	&M_{12} = M_{21} = m_2l_1l_{c2}\cos(\theta_2(t))+m_2l_{c2}^2+I_2,\notag \\
	&M_{22} = m_2l_{c2}^2+I_2,\notag
\end{align*}
\begin{align*}
	&C_{11} = -m_2l_1l_{c2}\sin(\theta_2(t))\dot{\theta}_2(t),\notag\\
	&C_{12} = -m_2l_1l_{c2}\sin(\theta_2(t))(\dot{\theta}_1(t)+\dot{\theta}_2(t)),\label{model_params}\\
	&C_{21} = m_2l_1l_{c2}\sin(\theta_2(t))\dot{\theta}_1(t),\notag\\
	&C_{22} = 0,\notag\\
	&g_{11} = m_1l_{c1}\textup{g}\cos(\theta_1(t)) + m_2\textup{g}(l_{c2}\cos(\theta_1(t)+\theta_2(t))\notag\\
	&\qquad\,+l_1\cos(\theta_1(t))),\notag\\
	&g_{21} = m_2l_{c2}\textup{g}\cos(\theta_1(t)+\theta_2(t)).\notag
\end{align*}
The true (unknown) parameters of the system are $m_1=m_2=1$\,kg, where $m$ denotes the mass of each pendulum and $l_1=l_2=0.5$\,m are their lengths. The moment of inertia of each rod around its center is denoted by $I_i=\frac{1}{12} m_i l_i^2$ with $l_{ci}=\frac{1}{2}l_i$ being the distance from the center of each rod to the actuated joint. The estimated model parameters are $\tilde{m}_1 = 1.0315$\,kg, $\tilde{m}_2 = 0.9627$\,kg, $\tilde{l}_1 = 0.5202$\,m, $\tilde{l}_2 = 0.5206$\,m.\par
The unmodeled dynamics are given by sigmoidal and cubic damping effects (cf. \cite{Gaz19}, where similar sigmoidal functions were used to model damping effects)
\begin{equation}
	f_u(t)=\begin{bmatrix}
		f_{u1}(t)\\ f_{u2}(t)
	\end{bmatrix} = \begin{bmatrix}
		0.1\frac{1-e^{-3\dot{\theta}_1}}{1+e^{-3\dot{\theta}_1}} - 0.1\dot{\theta}_1^3\\ 0.1\frac{1-e^{-3\dot{\theta}_2}}{1+e^{-3\dot{\theta}_2}} - 0.1\dot{\theta}_2^3
	\end{bmatrix}.
\end{equation}
%%%%%%%%%%%%%%

==> sections/DB_rep.tex <==
\section{Willems' Fundamental Lemma for Feedback Linearizable Systems}\label{DB_analysis_sec}
	Theorem \ref{MIMO_FL_thm} provided conditions under which the nonlinear system \eqref{NLsys} is feedback linearizable. Notice from \eqref{BINF} that if $\sum_i d_i = n$, then $\eta_k$ in \eqref{BINF_b} no longer exists and the system is {fully} feedback linearizable (i.e., both input-state and input-output maps are linearized). In particular, the system can be written as
	\begin{equation}
		\begin{aligned}
			\Xi_{k+1} &= \mathcal{A} \Xi_k + \mathcal{B}\mathbf{v}_k,\\
			\mathbf{y}_k &= \mathcal{C} \Xi_k.
		\end{aligned}
		\label{Lsys}
	\end{equation}
	\indent In this paper, we consider MIMO systems which are fully feedback linearizable\footnote{In \cite{Diwold22}, it was shown that for the SISO case, this condition (i.e., $d=n$) is satisfied if and only if the SISO system is flat. However, for MIMO systems, flatness is not a sufficient condition for full feedback linearizability (i.e., $\sum_i d_i=n$). Instead, fully feedback linearizable systems are a subclass of MIMO flat systems.} and can be expressed as in \eqref{Lsys}. Therefore, the following assumption will be made throughout the paper.
	\begin{assumption}\label{sum_di_asmp}
		The sum of relative degrees of the outputs of system \eqref{NLsys} is equal to the system dimension, i.e., $\sum_i d_i=n$.
	\end{assumption}
	In the setting of data-based control, one typically only has access to input-output data (i.e., $\mathbf{u}_k,\mathbf{y}_k$) and not the synthetic input $\mathbf{v}_k$ or the corresponding state transformation $\Xi_k = T_1(\mathbf{x}_k)$. In order to come up with a data-based description of the trajectories of the nonlinear system \eqref{NLsys} (or the equivalent system \eqref{Lsys}), we first express the synthetic input as\footnote{The invertibility of $\gamma(\mathbf{x}_k,\mathbf{v}_k)$ w.r.t. to $\mathbf{v}_k$ is guaranteed by Theorem \ref{MIMO_FL_thm}.} $\mathbf{v}_k = \Phi(\mathbf{u}_k,\mathbf{x}_k)\coloneqq\gamma^{-1}(\mathbf{x}_k,\mathbf{v}_k)$. It was shown in \cite{MonacoNor1987} that this inverse is in fact the iterated composition of the analytic functions $\boldsymbol{f}(\cdot,\cdot),\boldsymbol{h}(\cdot)$ in \eqref{NLsys} (hence it is locally Lipschitz continuous). Specifically,
	\begin{equation}
		\begin{aligned}
			\mathbf{v}_k &= \begin{bmatrix}
				v_{1,k} \\ \vdots \\ v_{m,k}
			\end{bmatrix} = \begin{bmatrix}
				{h}_1\left(\boldsymbol{f}_O^{d_1-1}\left(\boldsymbol{f}(\mathbf{x}_k,\mathbf{u}_k)\right)\right)\\
				\vdots\\
				{h}_m\left(\boldsymbol{f}_O^{d_m-1}\left(\boldsymbol{f}(\mathbf{x}_k,\mathbf{u}_k)\right)\right)
			\end{bmatrix}\\
			&\eqqcolon \begin{bmatrix}
				\phi_1(\mathbf{u}_k,\mathbf{x}_k)\\
				\vdots\\
				\phi_m(\mathbf{u}_k,\mathbf{x}_k)
			\end{bmatrix} = \Phi(\mathbf{u}_k,\mathbf{x}_k),
		\end{aligned}
		\label{definition_of_v_and_Phi}
	\end{equation}
	%For the remainder of this paper, $\mathbf{v}_k$ will be expressed as $\mathbf{v}_k= \Phi(\mathbf{u}_k,\Xi_k)$ with $\Phi:\mathbb{R}^m\times\mathbb{R}^n\to\mathbb{R}^m$.\par
%	\indent To obtain a data-driven representation of all the trajectories of \eqref{Lsys}, 
	\indent Since \eqref{definition_of_v_and_Phi} is \emph{unknown}, we approximate it by a suitable choice of basis functions that depend only on input-output data, since the state $\Xi_k$ consists of the shifted outputs as in \eqref{Xi}. In particular,
	% For the case of DT-SISO systems, we showed in our previous work \cite{AlsaltiBerLopAll2021} the special case where the nonlinear function $\Phi(\cdot,\cdot)$ is exactly decomposed using a linear combination of a finite number of bases functions. We use a set of basis functions that only depend on input-output data, since the state $\Xi_k$ consists of the shifted outputs as in \eqref{Xi}. In particular,
	\begin{equation}
		\begin{aligned}
			\mathbf{v}_k & = \Phi(\mathbf{u}_k,T_1^{-1}(\Xi_k)) = \begin{bmatrix}
				\phi_1(\mathbf{u}_k,\Xi_k)\\ \vdots \\ \phi_m(\mathbf{u}_k,\Xi_k)
			\end{bmatrix}\\
			&= \begin{bmatrix}
				\rule[.5ex]{1.5em}{0.4pt} \,g_1^\top\, \rule[.5ex]{1.5em}{0.4pt}\\
				\vdots\\
				\rule[.5ex]{1.5em}{0.4pt} \,g_m^\top\, \rule[.5ex]{1.5em}{0.4pt}\\
			\end{bmatrix}\Psi(\mathbf{u},\Xi_k) + \begin{bmatrix}
			\varepsilon_1(\mathbf{u}_k,\Xi_k)\\ \vdots\\ \varepsilon_m(\mathbf{u}_k,\Xi_k)
		\end{bmatrix}\\
			&\eqqcolon \mathcal{G}\Psi(\mathbf{u}_k,\Xi_k) + \scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k),
			\label{basis}
		\end{aligned}
	\end{equation}
%\footnote{Equation \eqref{def_of_G_mat} is not evaluated anywhere throughout the paper and it solely serves as a definition of $\mathcal{G}$.}
	where $\Psi(\mathbf{u}_k,\Xi_k)$ is the stacked vector of $r\in\mathbb{N}$ linearly independent basis functions $\psi_j(\mathbf{u}_k,\Xi_k):\mathbb{R}^m\times\mathbb{R}^n\to\mathbb{R}$ for $j\in\mathbb{Z}_{[1,r]}$ and $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ is the stacked vector of approximation errors $\varepsilon_i(\mathbf{u}_k,\Xi_k):\mathbb{R}^m\times\mathbb{R}^n\to\mathbb{R}$ for $i\in\mathbb{Z}_{[1,m]}$. The term $\mathcal{G}\in\mathbb{R}^{m\times r}$ is the matrix of unknown coefficients of the basis functions. For the theoretical analysis presented in this paper, we define, \emph{but never evaluate}, $\mathcal{G}$ as follows\footnote{The inner product is given by $\left< \rho_1(s_1,s_2), \rho_2(s_1,s_2) \right> = \int_\Omega \rho_1(s_1,s_2)\rho_2(s_1,s_2) ds_1 ds_2$ for some $\Omega\subseteq \mathbb{R}^m\times\mathbb{R}^n$.}
	\begin{equation}
%		\begin{aligned}
%			\mathcal{G}\coloneqq\argmin\limits_{\mathcal{G}} &\left< \Phi(s_1,s_2) \hspace{-0.5mm}-\hspace{-0.5mm} \mathcal{G}\Psi(s_1,s_2), \right.\\ &\left. \Phi(s_1,s_2) \hspace{-0.5mm}-\hspace{-0.5mm} \mathcal{G}\Psi(s_1,s_2) \right>.
%		\end{aligned}\label{def_of_G_mat}
		\mathcal{G}\hspace{-1mm}\coloneqq\hspace{-1mm}\argmin\limits_{\mathcal{G}}\hspace{-0.5mm} \left\langle  \Phi(\hspace{-0.35mm}s_1,s_2\hspace{-0.35mm}) \hspace{-0.5mm}-\hspace{-0.5mm} \mathcal{G}\Psi(\hspace{-0.35mm}s_1,s_2\hspace{-0.35mm}), \Phi(\hspace{-0.35mm}s_1,s_2\hspace{-0.35mm}) \hspace{-0.5mm}-\hspace{-0.5mm} \mathcal{G}\Psi(\hspace{-0.35mm}s_1,s_2\hspace{-0.35mm}) \right\rangle\hspace{-0.5mm} .\label{def_of_G_mat}
	\end{equation}
	\indent The minimization problem in \eqref{def_of_G_mat} is a least squares problem that minimizes the average approximation error in a region of the input-state space $\Omega\in\mathbb{R}^m\times\mathbb{R}^n$. Even though we will not be evaluating \eqref{def_of_G_mat} throughout the paper, we will later see in Lemma \ref{Lemma_G} that a solution exists and can be upper bounded. Furthermore, if the choice of basis functions contains $\Phi(\mathbf{u}_k,\Xi_k)$ in their span then a unique solution to \eqref{def_of_G_mat} exists and the results of \cite{AlsaltiBerLopAll2021} are retrieved. Finally, the following assumption is made on $\mathcal{G}$.
	\begin{assumption}\label{rank_assmp_G}
		The matrix of coefficients $\mathcal{G}$ has full row rank.
	\end{assumption}
	Assumption \ref{rank_assmp_G} is fulfilled if, e.g., the synthetic inputs $\mathbf{v}_k$ are decoupled which is true in many practical systems (e.g., robotic manipulators). Furthermore, this assumption is important since the right inverse of $\mathcal{G}$ is needed at different steps throughout the theoretical analysis. With that in mind, one can substitute \eqref{basis} back into \eqref{Lsys} to obtain
	\begin{equation}
		\begin{aligned}
			\Xi_{k+1} &= \mathcal{A}\Xi_k + \mathcal{B}\left(\mathcal{G}\Psi(\mathbf{u}_k,\Xi_k)+\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)\right),\\
			&=  \mathcal{A}\Xi_k + \mathcal{B}\mathcal{G}\left(\Psi(\mathbf{u}_k,\Xi_k)+E(\mathbf{u}_k,\Xi_k)\right),\\
			\mathbf{y}_k &= \mathcal{C}\Xi_k,
		\end{aligned}\label{Lsys2}
	\end{equation}
	where $E(\mathbf{u}_k,\Xi_k)\coloneqq \mathcal{G}^\dagger\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ and $\mathcal{G}^\dagger\coloneqq \mathcal{G}^\top(\mathcal{GG}^\top)^{-1}$ is a right inverse of $\mathcal{G}$.	For convenience, we introduce the following notation which will be used throughout the paper.
	\begin{equation}
			\begin{matrix}
			\hat{\Psi}_k(\mathbf{u},\Xi) \coloneqq \Psi(\mathbf{u}_k,\Xi_k), &
			\hat{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi) \coloneqq 	\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k), \\
			\hat{\varepsilon}_{i,k}(\mathbf{u},\Xi) \coloneqq 	\varepsilon_i(\mathbf{u}_k,\Xi_k), &
			\hat{E}_k(\mathbf{u},\Xi) \coloneqq E(\mathbf{u}_k,\Xi_k).
		\end{matrix}\label{imp_defs}
	\end{equation}
%	\begin{subequations}
%		\begin{align}
%			\begin{matrix}
%				\hat{\Psi}_k(\mathbf{u},\Xi) \coloneqq \Psi(\mathbf{u}_k,\Xi_k), &
%				\hat{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi) \coloneqq 	\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k), \\
%				\hat{\varepsilon}_{i,k}(\mathbf{u},\Xi) \coloneqq 	\varepsilon_i(\mathbf{u}_k,\Xi_k), &
%				\hat{E}_k(\mathbf{u},\Xi) \coloneqq E(\mathbf{u}_k,\Xi_k).
%			\end{matrix}\label{imp_defs_a}\\
%			\intertext{The following relationships are also important and will be used at various points throughout the paper}
%			\begin{matrix}
%				\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k) = \mathcal{G}E(\mathbf{u}_k,\Xi_k),  &
%				\hat{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi) = 	\mathcal{G}\hat{E}_k(\mathbf{u},\Xi), \\
%				\varepsilon_i(\mathbf{u}_k,\Xi_k) = g_i^\top E(\mathbf{u}_k,\Xi_k), &
%				\hat{\varepsilon}_{i,k}(\mathbf{u},\Xi) = g_i^\top \hat{E}_k(\mathbf{u},\Xi).
%			\end{matrix}\label{imp_defs_b}
%		\end{align}\label{imp_defs}
%	\end{subequations}%
	Using the notation in \eqref{imp_defs}, system \eqref{Lsys2} can now be written as
	\begin{equation}
		\begin{aligned}
			\Xi_{k+1} &= \mathcal{A} \Xi_k + \mathcal{B}\mathcal{G}\left(\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\right),\\
			\mathbf{y}_k &= \mathcal{C} \Xi_k.
			\label{Lsys3}
		\end{aligned}
	\end{equation}
	\begin{remark}
		Notice that the system in \eqref{Lsys3} represents $m$ SISO systems of the form% from $\mathbf{v}$ to $\mathbf{y}$. This means that every sub-system can be viewed as a standalone SISO system of the form
		\begin{equation}
			\begin{aligned}
				\xi_{i,k+1} &=  A_i\xi_{i,k} + B_ig_i^\top\left(\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_{k}(\mathbf{u},\Xi)\right),\\
				y_{i,k} &= C_i \xi_{i,k}.
			\end{aligned}\label{siso_rep}
		\end{equation}
	\end{remark}
	The following lemma shows that for the systems in \eqref{Lsys3}, the pair $(\mathcal{A,BG})$ is controllable.
	\begin{lemma}\label{lemma_controllable_pair}
		The pair $(\mathcal{A,BG})$ is a controllable pair.
	\end{lemma}
	\begin{proof}
		See Appendix \ref{app_controllable_pair}.
	\end{proof}
	Systems that are in the block-Brunovsky canonical form as in \eqref{Lsys} have two very appealing properties that will be extensively used throughout the paper. First, the state $\Xi_k$ is defined as the shifted outputs as in \eqref{Xi}. Second, the system is input-output decoupled from $\mathbf{v}_k$ to $\mathbf{y}_k$. This means that the $i-$th synthetic input at time $k$ is equal to the $i-$th output at time $k+d_i$, i.e.,
		\begin{align}
			y_{i,k+d_i} \stackrel{\eqref{output_k},\eqref{definition_of_v_and_Phi}}{=} v_{i,k} &= \phi_i(\mathbf{u}_k,\Xi_k)\label{y_for_proofs}\\
			&\stackrel{\eqref{siso_rep}}{=} g_i^\top\left(\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)\right)\notag.
		\end{align}
	\indent In the following theorem, we present the extension of the fundamental lemma to the class of DT-MIMO fully feedback linearizable nonlinear systems \eqref{NLsys} which have an equivalent linear representation in transformed coordinates \eqref{Lsys3}.
	\begin{theorem}\label{DB_MIMO_rep}
		Suppose Assumptions \ref{MIMO_img_assmp}--\ref{rank_assmp_G} are satisfied and let $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$, for $i\in\mathbb{Z}_{[1,m]}$, be a trajectory of a fully feedback linearizable system as in \eqref{NLsys}. Furthermore, let $\{\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ from \eqref{Lsys3} be persistently exciting of order $L+n$. Then, any $\{\mathbf{\bar{u}}_k\}_{k=0}^{L-1}$, $\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$ is a trajectory of system \eqref{NLsys} if and only if there exists $\alpha\in\mathbb{R}^{N-L+1}$ such that the following holds
		\begin{equation}
			\hspace{-3mm}\begin{bmatrix}\hspace{-0.5mm}
				H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{L+1}(\Xi)\end{bmatrix}\hspace{-0.5mm}\alpha \hspace{-0.25mm}=\hspace{-0.25mm} \begin{bmatrix}
				\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}
			\end{bmatrix}\hspace{-1mm},
			\label{inexact_result}
		\end{equation}
		where $\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})$ is the stacked vector of the sequence $\{\hat{\Psi}_k(\mathbf{\bar{u}},\bar{\Xi})+\hat{E}_k(\mathbf{\bar{u}},\bar{\Xi})\}_{k=0}^{L-1}$, while $\Xi,\,\bar{\Xi}$ are the stacked vectors of $\{\Xi_k\}_{k=0}^{N},\,\{\bar{\Xi}_k\}_{k=0}^{L}$ which, according to \eqref{Xi}, are composed of $\{y_{i,k}\}_{k=0}^{N+d_i-1},\,\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$, respectively.%, for $i\in\mathbb{Z}_{[1,m]}$.
	\end{theorem}
	\begin{proof}
		According to Theorem \ref{MIMO_FL_thm}, $\{\hat{\Psi}_k(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}_k(\mathbf{\bar{u}},\bar{\Xi})\}_{k=0}^{L-1}$, $\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$ is an input-output trajectory of \eqref{Lsys3} if and only if $\{\mathbf{\bar{u}}_k\}_{k=0}^{L-1},\,\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$ is an input-output trajectory of \eqref{NLsys}.\par
		%
		Using the input-output trajectory $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$ of system \eqref{NLsys}, one can construct the following sequences $\{\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ and $\{\Xi_k\}_{k=0}^{N}$ (using \eqref{basis} and \eqref{Xi}, respectively), which correspond to an input-state trajectory of the DT-LTI system in \eqref{Lsys3}. Since $\hat{\Psi}(\mathbf{u},\Xi)+\hat{E}(\mathbf{u},\Xi)$ is persistently exciting of order $L+n$ by assumption, and the pair $(\mathcal{A},\mathcal{B}\mathcal{G})$ is controllable by Lemma \ref{lemma_controllable_pair}, then \cite{Willems05} shows that any $\{\hat{\Psi}_k(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}_k(\mathbf{\bar{u}},\bar{\Xi})\}_{k=0}^{L-1},\,\{\bar{\Xi}_{k}\}_{k=0}^{L-1}$ is an input-state trajectory of \eqref{Lsys3} if and only if there exists $\alpha\in\mathbb{R}^{N-L+1}$ such that
		\begin{equation}
			\hspace{-3mm}\begin{bmatrix}\hspace{-0.5mm}
				H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ H_{L}(\Xi_{[0,N-1]})\end{bmatrix}\hspace{-0.5mm}\alpha \hspace{-0.25mm}=\hspace{-0.25mm} \begin{bmatrix}
				\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ \bar{\Xi}_{[0,L-1]}
			\end{bmatrix}\hspace{-1mm}.
			\label{NL_incomplete_willems_lemma}
		\end{equation}
		Next, notice from \eqref{y_for_proofs} that for each output $\bar{y}_i$, for $i\in\mathbb{Z}_{[1,m]}$, the following holds
		\begin{align}
			&\hspace{0mm}\bar{y}_{i,[L,L+d_i-1]}\label{last_di_outputs}\\ &\hspace{2mm}\stackrel{\eqref{y_for_proofs}}{=} g_i^\top\left(\hat{\Psi}_{[L-d_i,L-1]}(\mathbf{\bar{u}},\bar{\Xi})+\hat{E}_{[L-d_i,L-1]}(\mathbf{\bar{u}},\bar{\Xi})\right)\notag\\
			&\hspace{2mm}\stackrel{\eqref{NL_incomplete_willems_lemma}}{=} g_i^\top H_{d_i}\left(\hat{\Psi}_{[L-d_i,N-1]}(\mathbf{u},{\Xi})+\hat{E}_{[L-d_i,N-1]}(\mathbf{u},{\Xi})\right)\alpha\notag\\
			%\bar{y}_{i,[L,L+d_i-2]}
			&\hspace{2mm}\stackrel{\eqref{y_for_proofs}}{=} H_{d_i}\left(y_{i,[L,N+d_i-1]}\right)\alpha.\notag
		\end{align}
		Furthermore, the state $\bar{\Xi}_L$ can be written as
		\begin{align}
			\bar{\Xi}_L &\stackrel{\eqref{Xi}}{=} \begin{bmatrix}
				\bar{y}_{1,[L,L+d_1-1]} \\ \vdots \\ \bar{y}_{m,[L,L+d_m-1]}
			\end{bmatrix} \stackrel{\eqref{last_di_outputs}}{=} \begin{bmatrix}
			H_{d_1}(y_{1,[L,N+d_1-1]})\\ \vdots \\ H_{d_m}(y_{m,[L,N+d_m-1]})
		\end{bmatrix}\alpha\notag\\
		& = H_1(\Xi_{[L,N]})\alpha.\label{last_xi}
		\end{align}
	Therefore, concatenating \eqref{last_xi} with \eqref{NL_incomplete_willems_lemma} results in \eqref{inexact_result} which completes the proof.
	\end{proof}
	Theorem \ref{DB_MIMO_rep} extends the results of Theorem \ref{WFL} to general DT-MIMO feedback linearizable nonlinear systems of the form \eqref{NLsys}. This is done by exploiting linearity in transformed coordinates as shown in \eqref{Lsys} and using a dictionary of known basis functions which depend only on input-output data as in \eqref{basis}. However, the approximation error, $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$, is generally unknown in practice. Therefore, we present in the next sections a constructive method to use a data-based \emph{approximation} of DT-MIMO systems for data-driven simulation, output-matching control and predictive control problems despite unknown basis functions approximation error. %In particular, we will provide error bounds on approximate data-based predictions and their true counterparts in each of the two problems. Moreover, we later use such data-based approximation of the trajectories of the nonlinear system for data-driven nonlinear predictive control. Specifically, we propose a robust data-driven nonlinear predictive control scheme which is recursively feasible and renders the closed-loop equilibrium practically exponentially stable despite the inexact basis functions decomposition, similar to \cite{Berberich203}.
	%as in that the unknown nonlinear function $\mathbf{v}_k= \Phi(\mathbf{u}_k,\Xi_k)$ is approximated by a finite number of basis functions

==> sections/SIM_OM.tex <==
\section{Data-Driven Simulation \& Output-Matching}\label{sim_om_sec}
In this section, we investigate the data-driven simulation and output-matching control problems for the class of DT-MIMO feedback linearizable nonlinear systems \eqref{NLsys} using the results of Theorem \ref{DB_MIMO_rep}, as opposed to \cite{Rapisarda08, Berberich20} where the two problems were solved for DT-LTI systems. Compared to \cite{AlsaltiBerLopAll2021}, we consider the practically relevant setting where the chosen basis functions only approximate the unknown nonlinearities, i.e., $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)\not\equiv0$ for all $k\geq0$ in \eqref{basis}. Since this error is unknown, we provide a constructive method to approximate the solutions of the simulation and output matching problems and show that the difference between the approximate solutions and their true counterparts is bounded under the assumption that $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ is uniformly upper bounded.
%approximation error $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ in \eqref{basis} is unknown but uniformly upper bounded for all time. In particular, we show how the difference between the approximate solutions and their true counterparts can be upper bounded using reasonable assumptions on $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$.
%In this section, we provide a constructive method for obtaining approximate solutions for the data-based simulation and output matching problems, then show how the error between the approximate solutions and their true counterparts can be bounded using reasonable assumptions on ${E}(\mathbf{u}_k,\Xi_k)$. In the following sub-sections, we formally define these two problems first then modify Propositions 2 and 3 from \cite{AlsaltiBerLopAll2021} to match the current MIMO setting before finally showing the main results.
\subsection{Data-driven simulation}\label{sim_sec}
The data-driven simulation problem is defined as follows.
\begin{definition}\label{DD_sim_def}
	\textup{\textbf{Data-driven simulation}\cite{Rapisarda08}\textbf{:}}  Given an input $\mathbf{\bar{u}}$ and initial conditions $\bar{\mathbf{x}}_0$ for the nonlinear system in \eqref{NLsys}, find the corresponding output trajectory $\mathbf{\bar{y}}$ in a data-driven fashion, without explicitly identifying a model of the system.
\end{definition}
As in \eqref{basis}, we use a choice of basis functions that, in general, only approximates the unknown nonlinearities of the system. Therefore, $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$, and hence $\hat{E}_k(\mathbf{u},\Xi)$, are generally unknown. For completeness, we first formulate the simulation problem with the (unknown) approximation error. Afterwards, we present a key result where one can obtain an approximate solution to the simulation problem and provide an upper bound on the difference of this approximate solution from the true one.
\begin{theorem}\label{MIMO_sim_thm}
	Suppose Assumptions \ref{MIMO_img_assmp}--\ref{rank_assmp_G} are satisfied and let $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$, for $i\in\mathbb{Z}_{[1,m]}$, be a trajectory of a fully feedback linearizable system as in \eqref{NLsys}. Furthermore, assume that
	$\{\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ from \eqref{Lsys3} is persistently exciting of order \(L+n\) and let \(\{\mathbf{\bar{u}}_k\}_{k=0}^{L-1}\) be a new input to be simulated with $\bar{\Xi}_{0}=\begin{bmatrix}
		\bar{y}_{1,[0,d_1-1]}^\top & \dots & \bar{y}_{m,[0,d_m-1]}^\top
	\end{bmatrix}^\top$ specifying initial conditions for the state $\bar{\Xi}$ in \eqref{Lsys3}. Then there exists \(\alpha\in\mathbb{R}^{N-L+1}\) such that the following holds
	\begin{gather}
		\hspace{-30mm}\begin{bmatrix}\hspace{-0.5mm}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}\hspace{-0.5mm}\alpha \hspace{-0.25mm}=\label{unsolvable} \\
		\hspace{20mm} \begin{bmatrix}
			\hat{\Psi}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha) + \hat{E}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)\\ 	\bar{\Xi}_0
		\end{bmatrix}\notag
	\end{gather}
	where $\hat{\Psi}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)+\hat{E}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)$ is the stacked vector of the sequence $\{\hat{\Psi}_k(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)+\hat{E}_k(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)\}_{k=0}^{L-1}$, with each element defined as $\hat{\Psi}_k(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)+\hat{E}_k(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)\coloneqq\Psi(\mathbf{\bar{u}}_k,H_1(\Xi_{[k,k+N-L]})\alpha)+{E}(\mathbf{\bar{u}}_k,H_1(\Xi_{[k,k+N-L]})\alpha)$, and $\hat{\Psi}(\mathbf{u},{\Xi})$,\, $\hat{E}(\mathbf{u},\Xi)$,\,$\Xi,\,\bar{\Xi}$ are defined as in Theorem \ref{DB_MIMO_rep}. Finally, it holds that $\bar{\Xi} = H_{L+1}(\Xi)\alpha$ and  $\bar{y}_{i,[0,L+d_i-1]}=H_{L+d_i}(y_{i})\alpha$ for all $i\in\mathbb{Z}_{[1,m]}$.
\end{theorem}%\textup{h}_k(\Xi_{[k,k+N-L]})
\begin{proof}
	Since $\bar{\Xi}_{0}=\begin{bmatrix}
		\bar{y}_{1,[0,d_1-1]}^\top & \dots & \bar{y}_{m,[0,d_m-1]}^\top
	\end{bmatrix}^\top$ specifies the initial conditions for the state $\bar{\Xi}$ in \eqref{Lsys3}, it directly follows from Theorem \ref{DB_MIMO_rep} that there exists $\alpha\in\mathbb{R}^{N-L+1}$ such that the following holds
	\begin{equation}
		\hspace{-3mm}\begin{bmatrix}\hspace{-0.5mm}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}\hspace{-0.5mm}\alpha \hspace{-0.25mm}=\begin{bmatrix}
			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}_0
		\end{bmatrix}\label{subset_of_unsolvable}\hspace{-1mm}.
	\end{equation}
	This is true since \eqref{subset_of_unsolvable} is a subset of the equations in \eqref{inexact_result}. However, since $\bar{\Xi}$ on the right hand side of \eqref{subset_of_unsolvable} is unknown (in particular, it is composed of $\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$ which are unknown), we substitute $\bar{\Xi}=H_{L+1}(\Xi)\alpha$ (equivalently $\bar{y}_i = H_{L+d_i}(y_i)\alpha$ by \eqref{Xi}) which holds by Theorem \ref{DB_MIMO_rep}. This substitution results in the equivalent equation \eqref{unsolvable}.
\end{proof}
Notice that if $\hat{E}_k(\mathbf{u},\Xi)\equiv0$ for all $k\geq0$, i.e., if the nonlinear function $\Phi(\mathbf{u}_k,\Xi_k)$ in \eqref{basis} lies in the span of the chosen set of basis functions, then one can obtain a solution for $\alpha$ by solving the set of nonlinear equations \eqref{unsolvable} (cf. \cite[Proposition 2]{AlsaltiBerLopAll2021}, where the problem was cast as a nonlinear optimization problem). However, $\hat{E}(\mathbf{u},\Xi)$ is in general unknown, implying that one cannot directly use \eqref{unsolvable} to solve for $\alpha$. As an alternative, we propose in Theorem \ref{MIMO_inexact_sim_thm} a method to solve for an approximate simulated output (denoted $\hat{y}_{i}$ for $i\in\mathbb{Z}_{[1,m]}$) in a data-driven fashion using only data that is available a priori (namely $\{\mathbf{u}_k\}_{k=0}^{N-1},\{y_{i,k}\}_{k=0}^{N+d_i-1}$). Then, we derive upper bounds on the norm of their difference $e_i\coloneqq\bar{y}_i-\hat{y}_i$, where $\bar{y}_{i}$ is the actual response of the system \eqref{NLsys} to $\mathbf{\bar{u}}_{[0,L-1]}$. %To do so, we assume that the error in the basis function approximation $\varepsilon_i(\mathbf{u}_k,\Xi_k)$ is uniformly upper bounded, as stated in the following assumption.
To do so, in the following we restrict our analysis to a compact subset of the input-state space $\Omega\subseteq\mathbb{R}^m\times\mathbb{R}^n$, i.e., we assume from here on that the a priori collected trajectory as well as the simulated trajectory\footnote{Later in Theorem \ref{MIMO_inexact_om_thm}, we similarly assume that the matched trajectories evolve in a compact subset of the input-state space. For the robust nonlinear predictive control scheme in Section \ref{robust_nmpc_sec}, we prove in Theorem \ref{rob_npc_thm} that the closed-loop trajectories indeed evolve in a compact subset of the input-state space.} evolve in a compact set $\Omega$. This, along with local Lipschitz continuity of the function $\Phi(\mathbf{u}_k,\Xi_k)$ (cf. \eqref{definition_of_v_and_Phi} and the discussion above it), and assuming continuity of the chosen basis functions, guarantees a uniform upper bound on the approximation error $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ for all $(\mathbf{u}_k,\Xi_k)\in\Omega$. This assumption is summarized as follows.
\begin{assumption}\label{bounded_err_assmp}
	The error in the basis function approximation ${\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi)$ is uniformly upper bounded by $\varepsilon^*>0$, i.e., $\norm*{{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi)}_\infty\leq\varepsilon^*$, for all $(\mathbf{u}_k,\Xi_k)\in\Omega\subseteq\mathbb{R}^m\times\mathbb{R}^n$, where $\Omega$ is a compact subset of the input-state space.
\end{assumption}
%This assumption is satisfied if, for example, the inputs and outputs are contained in a compact set of the input-output space and the basis functions $\Psi(\cdot,\cdot)$ are continuous. Furthermore, this assumption implies that 
Recall that $E(\mathbf{u}_k,\Xi_k)\coloneqq \mathcal{G}^\dagger\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$, and hence, assumption \ref{bounded_err_assmp} implies
\begin{equation}
	\begin{aligned}
%	\norm*{\hat{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi)}_\infty&=\max_i{|\varepsilon_i(\mathbf{u}_k,\Xi_k)|}\leq\varepsilon^*,\\
		\norm*{\hat{E}_k(\mathbf{u},\Xi)}_\infty &{\leq} \norm*{\mathcal{G}^\dagger}_\infty\norm*{\hat{\scalebox{1.5}{$\epsilon$}}_k(\mathbf{u},\Xi)}_\infty\leq\norm*{\mathcal{G}^\dagger}_\infty\varepsilon^*.
	\end{aligned}\label{tilde_E_bdd_asmp}
\end{equation}
\indent In the following theorem, the idea is to use a modified version of \eqref{unsolvable} and solve a minimization problem for $\alpha$ instead of a set of nonlinear equations. Once a solution is obtained, an approximate output trajectory is given by $\bar{y}_{i,[0,L+d_i-1]}=H_{L+d_i}(y_{i})\alpha$, for all $i\in\mathbb{Z}_{[1,m]}$.
\begin{theorem}\label{MIMO_inexact_sim_thm}
	Suppose Assumptions \ref{MIMO_img_assmp}-\ref{bounded_err_assmp} are satisfied and let $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$, for $i\in\mathbb{Z}_{[1,m]}$, be a trajectory of a fully feedback linearizable system as in \eqref{NLsys}. Furthermore, let \(\{\mathbf{\bar{u}}_k\}_{k=0}^{L-1}\) be a new input to be simulated with \(\bar{\Xi}_0=\begin{bmatrix}
		\bar{y}_{1,[0,d_1-1]}^\top & \dots & \bar{y}_{m,[0,d_m-1]}^\top
	\end{bmatrix}^\top\) specifying initial conditions for the state $\bar{\Xi}$ in \eqref{Lsys3} and let the estimated simulated outputs of the system be defined as $\hat{y}_{i,[0,L+d_i-1]} = H_{L+d_i}(y_i)\alpha^*$ for $i\in\mathbb{Z}_{[1,m]}$, where
	\begin{subequations}
		\begin{align}
			\alpha^{*}\in&\argmin\limits_{\alpha}\; J(\alpha)\coloneqq \norm*{\mathcal{H}}_2^2 + \lambda_\alpha\varepsilon^*\norm*{\alpha}_2^2,\label{alpha*_a}\\
			&\textup{s.t. } \bar{\Xi}_0 = H_1(\Xi_{[0,N-L]})\alpha,\label{alpha*_b}
		\end{align}\label{alpha*}%
	\end{subequations}%
	with
	\begin{equation}
		\mathcal{H}\hspace{-0.5mm}\coloneqq
			H_L(\hat{\Psi}(\mathbf{u},\Xi))
		\alpha - 
			\hat{\Psi}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha),\label{H}
	\end{equation}
	and $\hat{\Psi}(\mathbf{u},\Xi),\,\hat{\Psi}(\mathbf{\bar{u}},H_{L+1}(\Xi)\alpha)$ as defined in Theorem \ref{MIMO_sim_thm}. If \eqref{alpha*_b} is feasible for the given $\bar{\Xi}_0$, then the error ${e}_{i}\vcentcolon=\bar{y}_{i}-{\hat{y}}_{i}$ satisfies $e_{i,[0,d_i-1]}=\mathbf{0}$ and is upper bounded by
	\begin{equation}
		|{{e}_{i,k+d_i}}|\leq \mathcal{P}^{k}(K_\Xi)\left(\varepsilon^*(1+\norm*{\alpha^*}_1) + \norm*{g_i}_1\sqrt{c^\top c}\right),\label{err_sim}
	\end{equation}
	for all $k\in\mathbb{Z}_{[0,L-1]}$, where $K_\Xi$ is the Lipschitz constant of $\Phi(\mathbf{u}_k,\Xi_k)$ w.r.t. $\Xi_k$ in the set $\Omega$. Moreover, $c^\top c=J(\alpha^*)-\lambda_{\alpha}\varepsilon^*\norm*{\alpha^*}_2^2$ and $\mathcal{P}^k(K_\Xi)$ is a polynomial in $K_\Xi$ of degree $k$ of the form $\mathcal{P}^k(K_\Xi)=(K_\Xi)^k + (K_\Xi)^{k-1} + \dots + K_\Xi + 1$.
\end{theorem}% on a compact set $\Omega\subseteq\mathbb{R}^m\times\mathbb{R}^n$ as in Assumption \ref{bounded_err_assmp}
\begin{proof}
%	First, notice that ${y}_{i,k+d_i}\stackrel{\eqref{y_for_proofs}}{=}v_{i,k} = h_i\left(\boldsymbol{f}_O^{d_i-1}\left(\boldsymbol{f}(\mathbf{x}_k,\mathbf{u}_k)\right)\right)$, for $i\in\mathbb{Z}_{[1,m]}$ and $k\in\mathbb{Z}_{[d_i,L+d_i-2]}$. Since ${v}_{i,k} \stackrel{\eqref{definition_of_v_and_Phi}}{=} \phi_i(\mathbf{u}_k,\Xi_k)$ is the composition of analytic functions, then $\phi_i(\cdot,\cdot)$ is (locally) Lipschitz continuous with $K_{\phi_i}^\Xi$ being the continuity constant in $\Xi$ as in the Theorem statement. Second, notice that \eqref{H} evaluated at $\alpha^*$ does not necessarily equal zero. Therefore,
%In the following, we denote by $\hat{\Xi}$ the stacked vector of the estimated sequence which is composed of $\{\hat{y}_{i,k}\}_{k=0}^{L+d_i-2}$, for all $i\in\mathbb{Z}_{[1,m]}$, as in \eqref{Xi}.	 
	By definition of $\alpha^*$ from \eqref{alpha*} and for some $c$ in the theorem statement, it holds that
	\begin{equation}
	H_L(\hat{\Psi}(\mathbf{u},\Xi))\alpha^* = \hat{\Psi}(\mathbf{\bar{u}},\overbrace{H_{L+1}(\Xi)\alpha^*}^{\hat{\Xi}\coloneqq})+ c.\label{sim_opt}
	\end{equation}
	The constraint in \eqref{alpha*_b} fixes the initial estimated state $\hat{\Xi}_0 \coloneqq H_1(\Xi_{[0,N-L]})\alpha = \bar{\Xi}_0$ and hence $e_{i,[0,d_i-1]}=\bar{y}_{i,[0,d_i-1]}-\hat{y}_{i,[0,d_i-1]} = \mathbf{0}$. Furthermore, each simulated output $i\in\mathbb{Z}_{[1,m]}$ takes the form $\hat{y}_{i,k+d_i}=H_1(y_{i,[k+d_i,k+d_i+N-L]})\alpha^*$, for all $k\in\mathbb{Z}_{[0,L-1]}$. Therefore, using \eqref{y_for_proofs}, one can write
	%\footnote{Notice that $\hat{\Xi}_{k-d_i}= \textup{h}_{k-d_i}(\Xi_{[k-d_i,k-d_i+N-L]})\alpha=\begin{bmatrix}\hat{y}_{1,[k-d_i,k-d_i+d_1-1]}^\top&\dots&\hat{y}_{m,[k-d_i,k-d_i+d_m-1]}^\top\end{bmatrix}^\top$.}
	%\footnote{The elements $v_{i,k}=\phi_i(\mathbf{u}_k,\Xi_k),\,i\in\mathbb{Z}_{[1,m]}$ are the entries of $\Phi(\mathbf{u}_k,\Xi_k)$. Further, we define the sequence of approximation errors as $\check{\varepsilon}_i(\mathbf{u,y})$ with $\check{\varepsilon}_{i,k}(\mathbf{u,y})\coloneqq\varepsilon_i(\mathbf{u}_k,\Xi_k)$.}\\&\quad
	\begin{align}
		\hat{y}_{i,k+d_i} &= g_i^\top H_1\Big(\hat{\Psi}_{[k,k+N-L]}(\mathbf{u},\Xi)
		+\hat{E}_{[k,k+N-L]}(\mathbf{u},\Xi)\Big)\alpha^*\notag
		\\&= g_i^\top H_1\left(\hat{\Psi}_{[k,k+N-L]}(\mathbf{u},\Xi)\right)\alpha^*\label{proof_sim}
		\\&\quad+ H_1\left(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi)\right)\alpha^*\notag
		\\&\stackrel{\eqref{sim_opt}}{=} g_i^\top{\Psi}(\mathbf{\bar{u}}_{k},\hat{\Xi}_{k}) \hspace{-0.5mm}+ \hspace{-0.5mm}g_i^\top c_{k}\hspace{-0.5mm}+\hspace{-0.5mm} H_1\hspace{-0.5mm}\left(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi)\right)\alpha^*\notag
		\\&\stackrel{\eqref{basis}}{=}\phi_i(\mathbf{\bar{u}}_{k},\hat{\Xi}_{k}) - \varepsilon_i(\mathbf{\bar{u}}_{k},\hat{\Xi}_{k}) + g_i^\top c_{k}\notag
		\\&\quad+ H_1\left(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi)\right)\alpha^*,\notag
	\end{align}
	where 
	\begin{equation}
		\begin{aligned}
			\hat{\Xi}_{k}&= H_1(\Xi_{[k,k+N-L]})\alpha^*\\
			&=\begin{bmatrix}\hat{y}_{1,[k,k+d_1-1]}^\top&\dots&\hat{y}_{m,[k,k+d_m-1]}^\top\end{bmatrix}^\top\hspace{-2mm},
		\end{aligned}\label{xihat}
	\end{equation}
	and $c_{k}$ is the $k-$th entry of the vector $c$. The actual unknown output of the system satisfies \eqref{Lsys3}, and hence, each output $\bar{y}_{k+d_i}$ for $i\in\mathbb{Z}_{[1,m]}$ and $k\in\mathbb{Z}_{[0,L-1]}$ can be written as
	\begin{equation*}
	\bar{{y}}_{i,k+d_i} \stackrel{\eqref{y_for_proofs}}{=} v_{i,k} = \phi_i(\mathbf{\bar{u}}_{k},\bar{\Xi}_{k}).
	\end{equation*}
	Therefore, the output error is
	\begin{align}
		e_{i,k+d_i} &= \phi_i(\mathbf{\bar{u}}_{k},\bar{\Xi}_{k}) - \phi_i(\mathbf{\bar{u}}_{k},\hat{\Xi}_{k}) + \varepsilon_i(\mathbf{\bar{u}}_{k},\hat{\Xi}_{k}) - g_i^\top c_{k}\notag \\
		&\quad- H_1\left(\hat{\varepsilon}_{i,[k,k+N-L]}(\mathbf{u},\Xi)\right)\alpha^*		\label{sim_e_vector}
	\end{align}
	The expression in \eqref{sim_e_vector} can be upper bounded by
	\begin{align}
		\hspace{-1mm}|{{e}_{i,k+d_i}}|\hspace{-0.5mm} &\leq\hspace{-0.5mm} K_\Xi \norm*{\bar{\Xi}_{k} \hspace{-0.5mm}-\hspace{-0.5mm} \hat{\Xi}_{k}}_\infty \hspace{-2.5mm}+ \hspace{-0.5mm}\varepsilon^*(1\hspace{-0.5mm}+\hspace{-0.5mm}\norm*{\alpha^*}_1\hspace{-0.5mm}) \hspace{-0.5mm} + \hspace{-0.5mm}\norm*{g_i}_1\hspace{-0.5mm}\sqrt{c^\top\hspace{-0.5mm} c},\label{sim_bnd_b4_recursion}
	\end{align}
	where the first two terms of \eqref{sim_e_vector} were bounded by Lipschitz continuity of $\phi_i(\cdot,\cdot)$, the third term was bounded by $\varepsilon^*$ as in Assumption \ref{bounded_err_assmp} and the fourth term was bounded by $\norm*{g_i^\top}_\infty\norm{c_{k}}_{\infty}\leq\norm*{g_i}_1\norm*{c}_\infty\leq\norm*{g_i}_1\sqrt{c^\top c}$. Finally the last term in \eqref{sim_e_vector} was bounded by $\varepsilon^*\norm*{\alpha^*}_1$.\par
	To arrive at \eqref{err_sim}, we continue the proof by induction. Let $k=0$, Equation \eqref{sim_bnd_b4_recursion} yields
	\begin{equation}
		\begin{aligned}
			|e_{i,d_i}| \hspace{-0.5mm} &\leq \hspace{-0.5mm} K_\Xi\norm*{\bar{\Xi}_0 - \hat{\Xi}_0}_\infty \hspace{-2mm}+ \varepsilon^*(1+\norm*{\alpha^*}) + \norm*{g_i}_1\sqrt{c^\top c}\\
			&= \varepsilon^*(1+\norm*{\alpha^*}) + \norm*{g_i}_1\sqrt{c^\top c},
		\end{aligned}\label{induction_base}
	\end{equation}
	since $\bar{\Xi}_0 = \hat{\Xi}_0$. Notice that \eqref{induction_base} has the form \eqref{err_sim} with $\mathcal{P}^0(K_\Xi)=1$. Next, for the induction step, assume that the following holds for some $k\in\mathbb{Z}_{[1,L-1]}$, all $\bar{k}\in\mathbb{Z}_{[0,k-1]}$ and all $i\in\mathbb{Z}_{[1,m]}$
	\begin{equation}
		|{{e}_{i,\bar{k}+d_i}}|\leq \mathcal{P}^{\bar{k}}(K_\Xi)\left(\varepsilon^*(1+\norm*{\alpha^*}_1) + \norm*{g_i}_1\sqrt{c^\top c}\right).\label{induction_step1}
	\end{equation}
%	\begin{equation}
%		|\hspace{-0.25mm}{{e}_{i,k+d_i\hspace{-0.15mm}-\hspace{-0.15mm}1}}\hspace{-0.25mm}|\hspace{-0.75mm}\leq\hspace{-0.75mm} \mathcal{P}^{(\hspace{-0.1mm}k\hspace{-0.1mm}-\hspace{-0.1mm}1\hspace{-0.1mm})}\hspace{-0.5mm}(\hspace{-0.15mm}K_\Xi\hspace{-0.15mm})\hspace{-0.5mm}\left(\hspace{-0.5mm}\varepsilon^*(1\hspace{-0.2mm}+\hspace{-0.2mm}\norm*{\alpha^*}_1)\hspace{-0.5mm} +\hspace{-0.5mm} \norm*{g_i}_1\sqrt{c^\top c}\hspace{-0.25mm}\right)\hspace{-1mm}.\label{induction_step1}
%	\end{equation}
	Since $\mathcal{P}^{\bar{k}}(K_\Xi)$ increases with increasing $\bar{k}$, this implies that the following bound on the previous error instances holds
	\begin{equation}
		\norm*{e_{i,[0,k+d_i-1]}}_\infty \hspace{-0.5mm} \leq \hspace{-0.75mm} \mathcal{P}^{(\hspace{-0.1mm}k\hspace{-0.1mm}-\hspace{-0.1mm}1\hspace{-0.1mm})}\hspace{-0.5mm}(\hspace{-0.15mm}K_\Xi\hspace{-0.15mm})\hspace{-0.5mm}\left(\hspace{-0.5mm}\varepsilon^*(1\hspace{-0.2mm}+\hspace{-0.2mm}\norm*{\alpha^*}_1)\hspace{-0.5mm} +\hspace{-0.5mm} \norm*{g_i}_1\sqrt{c^\top c}\hspace{-0.25mm}\right)\hspace{-1mm}.\label{induction_allk}
	\end{equation}
	Then, by \eqref{sim_bnd_b4_recursion}, we have
	\begin{align}
		|{{e}_{i,k+d_i}}| \hspace{-0.5mm}&\leq\hspace{-0.5mm} K_\Xi \norm*{\bar{\Xi}_{k}\hspace{-0.5mm} -\hspace{-0.5mm} \hat{\Xi}_{k}}_\infty \hspace{-1.5mm}+\hspace{-0.5mm} \varepsilon^*(1\hspace{-0.25mm}+\hspace{-0.25mm}\norm*{\alpha^*}_1\hspace{-0.25mm}) \hspace{-0.5mm}+\hspace{-0.5mm} \norm*{g_i}_1\sqrt{c^\top c}\notag\\
		\hspace{-1mm}&\stackrel{\eqref{Xi},\eqref{xihat}}{=}\hspace{-0.5mm} K_\Xi\norm*{\begin{bmatrix}
					e_{1,[k,k+d_1-1]} \\ \vdots \\ e_{m,[k,k+d_m-1]}
		\end{bmatrix}}_\infty\hspace{-3mm} +\hspace{-0mm}\varepsilon^*(1+\norm*{\alpha^*}_1)\notag\\
		&\quad + \norm*{g_i}_1\sqrt{c^\top c}.\label{induction_step2}
	\end{align}
	Inequality \eqref{induction_allk} implies that the elements of the first term on the RHS of \eqref{induction_step2} are bounded by
	\begin{align*}
		\norm*{e_{j,[k,k+d_j-1]}}_\infty \hspace{-0.5mm} \leq \hspace{-0.75mm} \mathcal{P}^{(\hspace{-0.1mm}k\hspace{-0.1mm}-\hspace{-0.1mm}1\hspace{-0.1mm})}\hspace{-0.5mm}(\hspace{-0.15mm}K_\Xi\hspace{-0.15mm})\hspace{-0.5mm}\left(\hspace{-0.5mm}\varepsilon^*(1\hspace{-0.2mm}+\hspace{-0.2mm}\norm*{\alpha^*}_1)\hspace{-0.5mm} +\hspace{-0.5mm} \norm*{g_i}_1\sqrt{c^\top c}\hspace{-0.25mm}\right)\hspace{-1mm}.
	\end{align*}
	Therefore,
	\begin{align}
		|e_{i,k+d_i}|&\stackrel{\eqref{induction_step2}}{\leq} K_{\Xi}\left(\mathcal{P}^{k-1}(K_{\Xi})\right)\left(\varepsilon^*(1+\norm*{\alpha})+ \norm*{g_i}_1\sqrt{c^\top c}\right)\notag\\
		&\quad+\varepsilon^*(1+\norm*{\alpha})+ \norm*{g_i}_1\sqrt{c^\top c}\\
		&= \mathcal{P}^{k}(K_\Xi)\left(\varepsilon^*(1+\norm*{\alpha^*}_1) + \norm*{g_i}_1\sqrt{c^\top c}\right)\notag,
	\end{align}
	as in \eqref{err_sim}, which completes the proof.
\end{proof}
%for all $k\in\mathbb{Z}_{[d_i,L+d_i-2]}$ 	Therefore it holds that
%\begin{equation*}
%	|{{e}_{i,k}}|\leq ,
%\end{equation*}
%In general, the choice of basis functions from \eqref{basis} do not necessarily have the nonlinear function $\mathbf{v}_k=\Phi(\mathbf{u}_k,\Xi_k)$ in their span. Even if that were the case, then Theorem \ref{MIMO_sim_thm} would still require persistency of excitation of the input signal $\hat{\Psi}(\mathbf{u},\Xi)+\hat{E}(\mathbf{u},\Xi)$, which is not easily satisfied as in the LTI case where the persistency of excitation assumption can be satisfied by suitable design of the input sequence \cite{vanWaarde22}.
%Theorem \ref{MIMO_inexact_sim_thm} provides an alternative method to approximate the solution of the simulation problem in a data-based fashion for general DT-MIMO nonlinear systems as in \eqref{NLsys}, \emph{without} requiring persistency of excitation of $\hat{\Psi}(\mathbf{u},\Xi)$.
Theorem \ref{MIMO_inexact_sim_thm} provides an approximate solution to the data-driven simulation problem by solving the optimization problem in \eqref{alpha*}, which, compared to Theorem \ref{MIMO_sim_thm}, does not require knowledge of the basis functions approximation error $\hat{E}(\mathbf{u},\Xi)$ but a uniform upper bound on it as in Assumption \ref{bounded_err_assmp}. To this end, we require that \eqref{alpha*} is feasible (i.e., the constraint \eqref{alpha*_b} can be satisfied). This is, e.g., the case if the conditions of Theorem \ref{MIMO_sim_thm} are satisfied, i.e., $\{\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ is persistently exciting of order $L+n$ (cf. \eqref{unsolvable}). However, persistency of excitation condition is \emph{not} necessary for feasibility of \eqref{alpha*_b} and hence is not necessarily required for Theorem \ref{MIMO_inexact_sim_thm}. In fact, feasibility of \eqref{alpha*} is given for any $\bar{\Xi}_0$ if $H_1(\Xi_{[0,N-L]})$ has full row rank, which can be easily checked given the a priori collected data $\{\Xi_k\}_{k=0}^{N}$ (which is given by $\{y_{i,k}\}_{k=0}^{N+d_i-1}$ for all $i\in\mathbb{Z}_{[1,m]}$).
Moreover, Theorem \ref{MIMO_inexact_sim_thm} provides error bounds on the approximation error, i.e., how far the estimated simulated outputs $\hat{y}_{i,[0,L+d_i-1]}$ deviate from the actual system response $\bar{y}_{i,[0,L+d_i-1]}$. Since the solution of \eqref{alpha*} appears in the error bound, we incentivize solutions with smaller norm using a regularization term as in \eqref{alpha*}, which depends on the approximation error bound $\varepsilon^*$.\par
It can be seen from \eqref{err_sim} that the error bound depends on $\norm*{g_i}_1$, which is the corresponding row of the unknown matrix of coefficients $\mathcal{G}$ in \eqref{basis}. In Section \ref{prior_model_knowledge_sec}, we show how one can compute an upper bound on $\norm*{g_i}_1$, based only on data, under certain assumptions. In general, the error bound \eqref{err_sim} can be conservative due to the use of Lipschitz arguments. In particular, the geometric series
\begin{equation*}
	\begin{aligned}
		\mathcal{P}^k(K_{\Xi}) &= (K_{\Xi})^k + \cdots + K_{\Xi} + 1= \frac{1-(K_{\Xi})^{k+1}}{1-K_{\Xi}},
	\end{aligned}
\end{equation*}
diverges for $K_{\Xi}>1$ but converges to $\frac{1}{1-K_{\Xi}}$ for $K_{\Xi}<1$, in which case the error bound in \eqref{err_sim} is uniformly upper bounded for all $k$. In contrast, the actual error $e_{i,k}$ can potentially be (much) smaller than \eqref{err_sim}, depending on the ``quality" of the a priori collected data and the choice of basis functions.\par
The following lemma establishes the important qualitative result that if $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ is persistently exciting, then the error bounds in \eqref{err_sim} (and hence the true error) go to zero as the approximation error bound $\varepsilon^*$ goes to zero. This lemma will be very useful in establishing recursive feasibility of the robust data-driven nonlinear predictive control scheme in Section \ref{robust_nmpc_sec}.
\begin{lemma}\label{lemma_eps_zero}
Suppose that the conditions of Theorem \ref{MIMO_inexact_sim_thm} hold and let $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ be persistently exciting of order $L+n$.
Then, as $\varepsilon^*\to0$, the error $e_{i,[0,L+d_i-1]}\to0$ as well.
\end{lemma}
\begin{proof}
%	See Appendix \ref{lemma_proof_app}.
	It can be seen from \eqref{err_sim} that, for each fixed $k$, the error bound goes to zero as $\varepsilon^*\to 0$ \emph{if} \textbf{(i)} $\norm*{\alpha^*}_1$ is bounded and \textbf{(ii)} $c^\top c\to0$ as $\varepsilon^*\to 0$. To show these two properties, we start by proposing a candidate solution for the optimization problem in \eqref{alpha*}. For sufficiently small $\varepsilon^*$, persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ implies that of $\{\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ of the same order. Therefore, the following choice $\bar{\alpha}$ is a feasible solution to \eqref{alpha*}
	\begin{equation}
		\hspace{-3mm}\bar{\alpha} = \hspace{-1mm}\begin{bmatrix}\hspace{-0.5mm}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}^{\dagger}\begin{bmatrix}
			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}_0
		\end{bmatrix}\hspace{-1mm}.\label{alpha_bar_definition}
	\end{equation}
	This holds since, given the assumed persistency of excitation condition, the pseudoinverse in \eqref{alpha_bar_definition} is in fact a right inverse of the matrix on the left hand side of \eqref{subset_of_unsolvable} (cf. \cite{Willems05}).
	By optimality, we have that $J(\alpha^*)\leq J(\bar{\alpha})$, or
	\begin{equation*}
		\begin{aligned}
			&\overbrace{\norm*{\hspace{-0.5mm}\begin{bmatrix}
						H_L(\hat{\Psi}(\mathbf{u},\Xi)) \\ H_1(\Xi_{[0,N-L]})
					\end{bmatrix}\alpha^* - \begin{bmatrix}
						\hat{\Psi}(\mathbf{\bar{u}},H_{L}(\Xi)\alpha^*) \\ \bar{\Xi}_0\end{bmatrix}\hspace{-0.5mm}}_2^2}^{\stackrel{\eqref{sim_opt}}{=}c^\top c}\hspace{-2mm}+ \hspace{0mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\\
			&\hspace{-1mm}\leq\hspace{-1mm}\norm*{\hspace{-0.5mm}\begin{bmatrix}
				H_L(\hat{\Psi}(\mathbf{u},\Xi)) \\ H_1(\Xi_{[0,N-L]})
			\end{bmatrix}\bar{\alpha} - \begin{bmatrix}
			\hat{\Psi}(\mathbf{\bar{u}},H_{L}(\Xi)\bar{\alpha}) \\ \bar{\Xi}_0\end{bmatrix}\hspace{-0.5mm}}_2^2\hspace{-2mm}+\hspace{-1mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.
		\end{aligned}
	\end{equation*}
	{Using} \eqref{alpha_bar_definition}, this can be rewritten as
	\begin{equation}
		c^\top c+ \hspace{-0.5mm}\lambda_\alpha\varepsilon^*\norm*{\alpha^*}_2^2\hspace{0.1mm}\leq\hspace{0.1mm}\norm*{\hspace{-0.5mm}
				\hat{E}(\mathbf{\bar{u}},\bar{\Xi})
			\hspace{-1mm}-\hspace{-1mm}
				H_{L}(\hat{E}(\mathbf{u},\Xi))
			\hspace{-0.15mm}\bar{\alpha}}_2^2\hspace{-1mm}+\hspace{-0.5mm} \lambda_\alpha\varepsilon^*\norm*{\bar{\alpha}}_2^2.\label{RHS_to_0}
	\end{equation}
	\indent It is clear that the right hand side of \eqref{RHS_to_0} goes to zero as $\hat{E}(\mathbf{u},\Xi)\to0$ (cf. \eqref{tilde_E_bdd_asmp}) {as long as $\norm*{\bar{\alpha}}_2$ is bounded}. As a result, the left hand side, which is a sum of two non-negative terms, goes to zero as well, implying point \textbf{(ii)} above. Hence, it is only left to show that $\norm*{\bar{\alpha}}_2$ is bounded.\par
	Recall from \eqref{alpha_bar_definition} that $\bar{\alpha}$ satisfies the following
	\begin{equation*}
		\hspace{-1mm}\begin{bmatrix}\hspace{-0.5mm}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi) + \hat{E}(\mathbf{u},\Xi))\\ 	H_{1}(\Xi_{[0,N-L]})\end{bmatrix}\bar{\alpha} = \begin{bmatrix}
			\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})\\ 	\bar{\Xi}_0
		\end{bmatrix},
	\end{equation*}
	which can be rewritten as
	\begin{gather}
		\hspace{-20mm}\left(\overbrace{\begin{bmatrix}H_{L}(\hat{\Psi}(\mathbf{u},\Xi))\\ H_{1}(\Xi_{[0,N-L]})\end{bmatrix}}^{\eqqcolon \Theta} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}H_{L}(\hat{E}(\mathbf{u},\Xi))\\ \boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta \Theta}\right) \bar{\alpha}\notag\\
		\hspace{15mm}=\left(\overbrace{\begin{bmatrix}\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi})\\ \bar{\Xi}_0 \end{bmatrix}}^{\eqqcolon \mu} \hspace{-1mm}+\hspace{-1mm} \overbrace{\begin{bmatrix}\hat{E}(\mathbf{\bar{u}},\bar{\Xi}) \\ \boldsymbol{0}\end{bmatrix}}^{\eqqcolon \Delta \mu}\right).\label{Golub}
	\end{gather}
	Notice that for a \emph{fixed} simulated trajectory $\mathbf{\bar{u}},\bar{\Xi}$, \eqref{Golub} represents a perturbed under-determined system of linear equations. Therefore, by applying results from perturbation theory of under-determined system \cite[Theorem 5.6.1]{Golub12}, it can be shown that
	\begin{equation}
		\frac{\norm*{\bar{\alpha}\hspace{-0.5mm}-\hspace{-0.5mm}\alpha_{\textup{bnd}}}_2}{\norm*{\alpha_{\textup{bnd}}}_2}\hspace{-0.5mm}\leq\hspace{-0.5mm}\kappa_2(\Theta)\hspace{-0.5mm}\left(\hspace{-0.5mm}c_0\frac{\norm*{\Delta \Theta}_2}{\norm*{\Theta}_2} \hspace{-0.5mm}+\hspace{-0.5mm} \frac{\norm*{\Delta \mu}_2}{\norm*{\mu}_2}\hspace{-0.5mm}\right)\hspace{-0.5mm} +\hspace{-0.5mm} O(\sigma^2),\label{pertb_lin_sys}
	\end{equation}
	where $\alpha_{\textup{bnd}}=\Theta^\dagger \mu$ is the \textit{bounded} minimum-norm solution of the unperturbed system of equations\footnote{By Theorem \ref{WFL}, persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ implies that $\Theta+\Delta\Theta$ has full row rank. For sufficiently small $\varepsilon^*$, $\Theta$ also has full row rank and, hence, the unperturbed system of equations also has a solution.} and $\kappa_2(\Theta)=\norm*{\Theta}_2\norm*{\Theta^\dagger}_2$ is the condition number of the matrix $\Theta$. Moreover,\footnote{$n_{c,\Theta},\,n_{r,\Theta}$ are the numbers of columns and rows of matrix $\Theta$, respectively.} $c_0\coloneqq\min{\left\lbrace2, n_{c,\Theta}-n_{r,\Theta}+1\right\rbrace}$ and $\sigma\coloneqq\max{\left\lbrace\frac{\norm*{\Delta \Theta}_2}{\norm*{\Theta}_2},\frac{\norm*{\Delta \mu}_2}{\norm*{\mu}_2}\right\rbrace}$.\par
	From \eqref{Golub}, it can be seen that as $\varepsilon^*\to0$, the terms $\Delta\Theta,\,\Delta\mu\to0$ and, by \eqref{pertb_lin_sys}, the candidate $\bar{\alpha}$ approaches the bounded solution $\alpha_{\textup{bnd}}$, which is finite for any fixed $\mathbf{\bar{u}},\bar{\Xi}$. Therefore, the right hand side of \eqref{RHS_to_0} approaches zero as $\varepsilon^*\to 0$ and consequently, the left hand side does as well, which completes the proof.
\end{proof}
Lemma \ref{lemma_eps_zero} shows that the error bound in \eqref{err_sim}, and, hence, the true error between the results of Theorems \ref{MIMO_sim_thm} and \ref{MIMO_inexact_sim_thm}, go to zero as $\varepsilon^*$ goes to zero if persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ is satisfied. This condition can be checked after collecting the input-output data, but can, in general, not be enforced a priori by suitable design of the input sequence as it is the case for DT-LTI systems (cf. \cite{vanWaarde22}). Studying conditions on $\{\mathbf{u}_k\}_{k=0}^{N-1}$ that result in persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ for certain choices of basis functions and/or classes of unknown nonlinearities will be a topic of future research.
%In the following subsection, we investigate the data-driven output matching control problem and provide similar results to Theorems \ref{MIMO_sim_thm} and \ref{MIMO_inexact_sim_thm}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data-driven output-matching}\label{om_sec}
The data-driven output matching control problem is the dual problem of the simulation problem and is defined as follows.
\begin{definition}\label{DD_om_def}
	\textup{\textbf{Data-driven output-matching control}\cite{Rapisarda08}\textbf{:}} Given a desired reference trajectory $\mathbf{\bar{y}}$ and a corresponding initial condition $\bar{\mathbf{x}}_0$ for the nonlinear system in \eqref{NLsys}, find the required input trajectory $\mathbf{\bar{u}}$ that, when applied to the system, results in an output that tracks the desired reference trajectory, in a data-driven fashion.
\end{definition}
Analogous to the discussion in Section \ref{sim_sec}, we propose to solve the data-driven output matching problem for general DT-MIMO feedback linearizable nonlinear systems as in \eqref{NLsys}. Before presenting the result, the following assumption is made.
\begin{assumption}\label{u_in_span_asmp}
	Let $\mathbf{u}_k$ be one of the elements of $\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)$, i.e.,
	\begin{equation*}
		\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi) = \begin{bmatrix}
			\mathbf{u}_k\\ \psi_{m+1}(\mathbf{u}_k,\Xi_k) + \hat{e}_{m+1}(\mathbf{u}_k,\Xi_k) \\ \vdots \\ \psi_{r}(\mathbf{u}_k,\Xi_k) + \hat{e}_{r}(\mathbf{u}_k,\Xi_k)
		\end{bmatrix},
	\end{equation*}
	where $r>m$ and $\hat{e}_i(\mathbf{u}_k,\Xi_k)$ is the $i-$th entry of the vector $\hat{E}_k(\mathbf{u},\Xi)$.
\end{assumption}
Assumption \ref{u_in_span_asmp} is not very restrictive and is needed in order to retrieve the desired input $\mathbf{\bar{u}}$. It can also be replaced by only requiring $\mathbf{u}_k$ to lie in the span of $\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)$, which is not shown here for notational convenience.
%Assumption \ref{u_in_span_asmp} is not very restrictive since it is also sufficient that $\mathbf{u}_k$ is only in the span of $\hat{\Psi}_k(\mathbf{u},\Xi)+\hat{E}_k(\mathbf{u},\Xi)$. For brevity, this is not shown here.
The following theorem is the dual result of Theorem \ref{MIMO_sim_thm}.% and an extension of \cite[Proposition 3]{AlsaltiBerLopAll2021} to the MIMO setting.
\begin{theorem}\label{MIMO_om_thm}
	Suppose Assumptions \ref{MIMO_img_assmp}--\ref{rank_assmp_G} and \ref{u_in_span_asmp} are satisfied and let $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$, for $i\in\mathbb{Z}_{[1,m]}$, be a trajectory of a fully feedback linearizable system as in \eqref{NLsys}. Furthermore, let	$\{\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ from \eqref{Lsys3} be persistently exciting of order \(L+n\) and let \(\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}\) be the desired output reference trajectories with $\bar{\Xi}_{0}=\begin{bmatrix}
		\bar{y}_{1,[0,d_1-1]}^\top & \dots & \bar{y}_{m,[0,d_m-1]}^\top
	\end{bmatrix}^\top$ specifying initial conditions for the state $\bar{\Xi}$ in \eqref{Lsys3}. Then, there exists \(\alpha\in\mathbb{R}^{N-L+1}\) such that the following holds
	\begin{gather}
		\hspace{-30mm}\begin{bmatrix}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi)+\hat{E}(\mathbf{u},\Xi))\\ H_{L+1}(\Xi)
		\end{bmatrix}\alpha = \label{om_unsolvable} \\
		\hspace{20mm}\begin{bmatrix}
			\hat{\Psi}(H_{L}(\mathbf{u})\alpha,\bar{\Xi}) + \hat{E}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})\\ \bar{\Xi}
		\end{bmatrix}\notag,
	\end{gather}
	where $\hat{\Psi}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})+\hat{E}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})$ is the stacked vector of the sequence $\{\hat{\Psi}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})+\hat{E}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})\}_{k=0}^{L-1}$, with each element defined as $\hat{\Psi}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})+\hat{E}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})=\Psi(H_1(\mathbf{u}_{[k,k+N-L]})\alpha,\bar{\Xi}_{k})+{E}(H_1(\mathbf{u}_{[k,k+N-L]})\alpha,\bar{\Xi}_{k})$, and $\hat{\Psi}(\mathbf{u},{\Xi})$,\, $\hat{E}(\mathbf{u},\Xi)$,\,$\Xi,\,\bar{\Xi}$ are defined as in Theorem \ref{DB_MIMO_rep}. Finally, it holds that $\mathbf{\bar{u}}=H_{L}(\mathbf{u})\alpha$.
%	holds, where $\hat{\Psi}(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})$, $\hat{E}(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})$ are the stacked vectors of the sequences $\{\hat{\Psi}_k(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})\}_{k=0}^{L-d_q-1}$ and $\{\hat{E}_k(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})\}_{k=0}^{L-d_q-1}$ respectively, with $\hat{\Psi}_k(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})=\Psi(\textup{h}_k(\mathbf{u}_{[k,k+N-L]})\alpha,\bar{\Xi}_{k})$ and $\hat{E}_k(H_{L-d_q}(\mathbf{u})\alpha,\mathbf{\bar{y}})=\tilde{E}(\textup{h}_k(\mathbf{u}_{[k,k+N-L]})\alpha,\bar{\Xi}_{k})$, whereas $\hat{\Psi}(\mathbf{u,y})$ and $\hat{E}(\mathbf{u,y})$ are defined as in Theorem \ref{DB_MIMO_rep}. Finally, it holds that $\mathbf{\bar{u}}=H_{L-d_q}(\mathbf{u})\alpha$.
\end{theorem}
\begin{proof}
	Since $\bar{\Xi}_0$ specifies the initial condition for the state $\bar{\Xi}$ in \eqref{Lsys3}, it can be seen that any output reference trajectory $\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}$ is a trajectory of \eqref{NLsys} given $\bar{\mathbf{x}}_0 = T_1^{-1}(\bar{\Xi}_0)$, by choosing a suitable input sequence. In particular, since $\bar{y}_{i,k+d_i}\stackrel{\eqref{y_for_proofs}}{=}\phi_i(\mathbf{\bar{u}}_k,\bar{\Xi}_k)$ holds for $k\in\mathbb{Z}_{[0,L-1]}$ as in \eqref{Lsys}, then according to Theorem \ref{MIMO_FL_thm}, the required input to achieve the desired outputs is given by
%	\footnote{Recall that the transformation $T(\cdot)$ is invertible as in Theorem \ref{MIMO_FL_thm}. Moreover, with a slight abuse of notation, we use $\mathbf{\bar{v}}_k=\Phi(\mathbf{\bar{u}}_k,\bar{\Xi}_k)$}
	$\mathbf{\bar{u}}_k=\gamma(T_1^{-1}(\bar{\Xi}_k),\bar{\mathbf{v}}_k)$, where $\bar{v}_{i,k}=\bar{y}_{i,k+d_i}$ (cf. \eqref{y_for_proofs}).
	By persistency of excitation of $\{\hat{\Psi}_k(\mathbf{u},\Xi) + \hat{E}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$, it follows from Theorem \ref{DB_MIMO_rep} that there exists $\alpha\in\mathbb{R}^{N-L+1}$ such that \eqref{inexact_result} holds. However, since $\mathbf{\bar{u}}$ is unknown, we substitute $\mathbf{\bar{u}}=H_{L}(\mathbf{u})\alpha$. This can be done since by Theorem \ref{DB_MIMO_rep} it also holds that $\hat{\Psi}(\mathbf{\bar{u}},\bar{\Xi}) + \hat{E}(\mathbf{\bar{u}},\bar{\Xi})=H_{L}(\hat{\Psi}(\mathbf{u},{\Xi}) + \hat{E}(\mathbf{u},\Xi))\alpha$ and, hence, Assumption \ref{u_in_span_asmp} implies that $\mathbf{\bar{u}}=H_{L}(\mathbf{u})\alpha$. With this substitution into \eqref{inexact_result}, we obtain the equivalent equation \eqref{om_unsolvable}.
\end{proof}
Similar to Theorem \ref{MIMO_sim_thm}, notice that if $\hat{E}_k(\mathbf{u},\Xi)\equiv0$ for all $k\geq0$, one can obtain a solution for $\alpha$ by solving the set of nonlinear equations \eqref{om_unsolvable} (cf. \cite[Proposition 3]{AlsaltiBerLopAll2021}). However, for the more practical case which is considered throughout this paper, the approximation error $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$ is, in general, unknown. For that, we propose a similar approach to the one shown in Theorem \ref{MIMO_inexact_sim_thm} for solving the data-based output-matching control problem despite an unknown basis function approximation error and using only input-output data (namely $\{\mathbf{u}_k\}_{k=0}^{N-1},\{y_{i,k}\}_{k=0}^{N+d_i-1}$). In particular, we assume that the a priori collected data and the trajectory to be matched evolve in a compact subset of the input-state space as in Assumption \ref{bounded_err_assmp}. Next, we solve for an approximate control input $\hat{\mathbf{u}}_{[0,L-1]}$ that, when applied to the system, results in approximate output trajectories $\hat{y}_{i,[0,L+d_i-1]}$ which track the given reference trajectories $\bar{y}_{i,[0,L+d_i-1]}$ as closely as possible. The error between the two outputs is bounded as shown in the following theorem, which is the dual result to Theorem \ref{MIMO_inexact_sim_thm}.
\begin{theorem}\label{MIMO_inexact_om_thm}
	Suppose Assumptions \ref{MIMO_img_assmp}--\ref{u_in_span_asmp} are satisfied and let $\{\mathbf{u}_k\}_{k=0}^{N-1}$, $\{y_{i,k}\}_{k=0}^{N+d_i-1}$, for $i\in\mathbb{Z}_{[1,m]}$, be a trajectory of a fully feedback linearizable system as in \eqref{NLsys}. Furthermore, let \(\{\bar{y}_{i,k}\}_{k=0}^{L+d_i-1}\) be desired reference trajectories with \(\bar{\Xi}_0=\begin{bmatrix}
		\bar{y}_{1,[0,d_1-1]}^\top & \dots & \bar{y}_{m,[0,d_m-1]}^\top
	\end{bmatrix}^\top\) specifying the initial condition for the state $\bar{\Xi}$ in \eqref{Lsys3} and let $\hat{\mathbf{u}}\coloneqq H_{L}(\mathbf{u})\alpha^*$ be the estimated input to the system that, when applied to \eqref{NLsys}, results in the approximate outputs $\hat{y}_{i,[0,L+d_i-1]}$, for $i\in\mathbb{Z}_{[1,m]}$, where 
	\begin{subequations}
		\begin{align}
			\alpha^{*}\in&\argmin\limits_{\alpha}\; J(\alpha)\coloneqq \norm*{\mathcal{H}}_2^2 + \lambda_\alpha\varepsilon^*\norm*{\alpha}_2^2,\label{alpha*2_a}\\
			&\textup{s.t. } \bar{\Xi}_0 = H_1(\Xi_{[0,N-L]})\alpha,\label{alpha*2_b}
		\end{align}\label{alpha*2}%
	\end{subequations}%
	with
	\begin{equation}
		\mathcal{H}\coloneqq\begin{bmatrix}
			H_{L}(\hat{\Psi}(\mathbf{u},\Xi))\\ H_{L+1}(\Xi)
		\end{bmatrix}\alpha - \begin{bmatrix}
			\hat{\Psi}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})\\ \bar{\Xi}
		\end{bmatrix},\label{H2}
	\end{equation}
%, whereas $\hat{\Psi}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})$ is the stacked vector of the sequence $\{\hat{\Psi}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})\}_{k=0}^{L-1}$ with $\hat{\Psi}_k(H_{L}(\mathbf{u})\alpha,\bar{\Xi})=\Psi(H_1(\mathbf{u}_{[k,k+N-L]})\alpha,\bar{\Xi}_k)$
	and $\hat{\Psi}(\mathbf{u},\Xi),\,\hat{\Psi}(H_{L}(\mathbf{u})\alpha,\bar{\Xi})$ defined as in Theorem \ref{MIMO_om_thm}. If \eqref{alpha*2_b} is feasible for the given $\bar{\Xi}_0$, then the error ${e}_{i}\vcentcolon=\bar{y}_{i}-\hat{y}_{i}$ satisfies $e_{i,[0,d_i-1]}=\mathbf{0}$ and is upper bounded by
	\begin{equation}\hspace{-3mm}
		|{{e}_{i,k+d_i}}|\hspace{-0.5mm}\leq\hspace{-0.5mm} \mathcal{P}^{k}(K_\Xi)\hspace{-0.5mm}\left(\hspace{-0.5mm}\varepsilon^*(1\hspace{-0.5mm}+\hspace{-0.5mm}\norm*{\alpha^*}_1\hspace{-0.5mm})\hspace{-0.5mm} +\hspace{-0.5mm} (\norm*{g_i}_1\hspace{-0.5mm}+\hspace{-0.5mm}1)\sqrt{c^\top c}\right)\hspace{-1mm},\label{err_om}
	\end{equation}
	for all $k\in\mathbb{Z}_{[0,L-1]}$, where $K_\Xi$ is the Lipschitz continuity constant of $\Phi(\mathbf{u}_k,\Xi_k)$ w.r.t. $\Xi_k$ in the set $\Omega$, $c^\top c=J(\alpha^*)-\lambda_{\alpha}\varepsilon^*\norm*{\alpha^*}_2^2$ and $\mathcal{P}^k(K_\Xi)$ defined as in Theorem \ref{MIMO_inexact_sim_thm}.
\end{theorem}
\begin{proof}
	The proof follows similar steps as the proof of Theorem \ref{MIMO_inexact_sim_thm} and can be found in Appendix \ref{proof_om_app}.
\end{proof}
We have shown in Theorem \ref{MIMO_inexact_om_thm} how an approximate solution to the data-based output-matching control problem can be obtained despite the unknown, but uniformly upper bounded, basis function approximation error $\scalebox{1.5}{$\epsilon$}(\mathbf{u}_k,\Xi_k)$.\par
The error bound shown in \eqref{err_om} shares many features to that shown in \eqref{err_sim}. For instance, it increases with increasing $k$ (i.e., for longer matched output sequences). The bound can be conservative as well, especially for $K_\Xi>1$. However, it shows the same important qualitative behavior for vanishing approximation error. In particular, the error bound goes to zero as $\varepsilon^*\to0$ {and} if persistency of excitation condition of $\{\hat{\Psi}_k(\mathbf{u},\Xi)\}_{k=0}^{N-1}$ of order $L+n$ is satisfied. This can be shown for \eqref{err_om} using similar arguments as in Lemma \ref{lemma_eps_zero}.% (see Appendix \ref{lemma_eps_zero_OM}).
\subsection{Data-driven bounds on $\norm*{\mathcal{G}}$}\label{prior_model_knowledge_sec}
%In Theorems \ref{MIMO_inexact_sim_thm} and \ref{MIMO_inexact_om_thm}, we derived upper bounds on the difference between the approximate and actual solutions of the data-driven simulation and output matching problems, respectively. These bounds can be conservative due to their recursive nature (i.e., increasing bound with increasing sequence length). However, in practice one often has additional prior knowledge on the system under consideration (cf. e.g., \cite{BerberichModelKnowledge} where data-driven approaches were combined with prior model knowledge).
In this subsection, we show how an upper bound on $\norm*{g_i}_1$ can be obtained without model knowledge, which is required in order to evaluate the error bounds \eqref{err_sim} and \eqref{err_om}. To this end, recall that the system trajectories evolve in a compact subset of the input-state space $\Omega\subseteq\mathbb{R}^m\times\mathbb{R}^n$ (cf. Assumption \ref{bounded_err_assmp}). In such a compact set, the outputs (and hence the synthetic inputs) are uniformly bounded as follows
\begin{equation}
	|y_{i,k}| \stackrel{\eqref{y_for_proofs}}{=} |\phi_i(\mathbf{u}_{k+d_i},\Xi_{k+d_i})| \stackrel{\eqref{definition_of_v_and_Phi}}{=} |v_{i,k+d_i}|\leq v_i^*,\label{bounded_outputs_for_Gbnd}
\end{equation}
for some $v_{i}^*>0$, $i\in\mathbb{Z}_{[1,m]}$ and all $k\geq0$. To obtain an upper bound on $\norm*{g_i}_1$, we use \eqref{bounded_outputs_for_Gbnd} along with a possible method to solve \eqref{def_of_G_mat}. The following lemma summarizes this result.
% Although we do not explicitly evaluate the matrix $\mathcal{G}$ throughout the paper, inspecting a method of evaluating $\mathcal{G}$ will be insightful to get an upper bound on it.
\begin{lemma}\label{Lemma_G}
	Suppose Assumptions \ref{MIMO_img_assmp}--\ref{bounded_err_assmp} hold and let the basis functions $\psi_j$ be chosen such that the symmetric matrix of their inner products is invertible, i.e., det$(\Gamma)\neq0$ with $\Gamma_{j,\ell}=\left\langle \psi_j,\psi_\ell\right\rangle$. Then, the following holds
	%the norm of the matrix $\mathcal{G}$ can be upper bounded by
	\begin{equation}
		\hspace{-2mm}\norm*{g_i}_1 \hspace{-0.75mm} =\hspace{-0.75mm} \norm*{g_i^\top}_\infty \hspace{-0.75mm}\leq\hspace{-0.75mm} v_i^* \norm*{\Gamma^{-1}}_1\hspace{-1mm} \sum\limits_{j=1}^r\hspace{-0.5mm}\int_{\Omega}\hspace{-1mm}\left|{\psi}_j(s_1,s_2)\right|ds_1ds_2.		\label{G_bnd_a}
	\end{equation}
\end{lemma}
\begin{proof}
	Each row of the matrix $\mathcal{G}$, i.e., $g_i^\top$ is defined as
	\begin{align}
%		g_i \hspace{-0.25mm}\stackrel{\eqref{def_of_G_mat}}{=}\hspace{-0.25mm} &\argmin\limits_{g_i}&&\hspace{-3mm}\left<\hspace{-0.5mm} \phi_{i}(s_1,s_2)\hspace{-0.5mm}-\hspace{-0.5mm}g_i^\top{\Psi}(s_1,s_2),\phi_{i}(s_1,s_2)\hspace{-0.5mm}-\hspace{-0.5mm}g_i^\top{\Psi}(s_1,s_2) \hspace{-0.5mm}\right>\notag\\
		g_i \hspace{-0.25mm}\stackrel{\eqref{def_of_G_mat}}{=}\hspace{-0.25mm}		&\argmin\limits_{g_i}&&\hspace{-3mm}\left< \phi_{i}(s_1,s_2),\phi_{i}(s_1,s_2)\right>\notag\\[-1ex]
		& &&\hspace{-3mm}- 2\left<\phi_{i}(s_1,s_2),g_i^\top{\Psi}(s_1,s_2)\right>\label{min_for_g}\\
		& &&\hspace{-3mm}+\left< g_i^\top{\Psi}(s_1,s_2),g_i^\top{\Psi}(s_1,s_2)\right>.\notag
	\end{align}
	Since $\Gamma$ is assumed to be invertible, Equation \eqref{min_for_g} represents a least squares problem whose unique solution can be obtained by the following linear system of equations $\Gamma {g_i} = \zeta$, where
	\begin{equation*}
		\begin{aligned}
		\Gamma_{j,\ell} &= \left<{\psi}_j(s_1,s_2),{\psi}_\ell(s_1,s_2)\right>,\\ \zeta_{j} &= \left<\phi_i(s_1,s_2),{\psi}_j(s_1,s_2)\right>.%\label{gamma_mat}
		\end{aligned}
	\end{equation*}
%	and $\psi_j$ being the individual basis functions in $\Psi(s_1,s_2)$ as in \eqref{basis}. 
	In particular, the solution to \eqref{min_for_g} takes the form
	\begin{equation*}
		\begin{aligned}
			g_i &= \Gamma^{-1}\zeta,\\
			\norm*{g_i^\top}_\infty = \norm{g_i}_1 &\leq \norm{\Gamma^{-1}}_1 \norm{\zeta}_1.
		\end{aligned}
	\end{equation*}
	Moreover, using the definition of $\zeta$, we write
	\begin{equation*}
		\begin{aligned}
		\norm{\zeta}_1 &= \norm*{\begin{bmatrix}
				\int_{\Omega}\phi_i(s_1,s_2){\psi}_1(s_1,s_2)ds_1ds_2\\
				\vdots\\
				\int_{\Omega}\phi_i(s_1,s_2){\psi}_r(s_1,s_2)ds_1ds_2\\
		\end{bmatrix}}_1\\
		&= \sum\limits_{j=1}^r\left|\int_{\Omega}\phi_i(s_1,s_2){\psi}_j(s_1,s_2)ds_1ds_2\right|\\
		&\leq\sum\limits_{j=1}^r\int_{\Omega}\left|\phi_i(s_1,s_2){\psi}_j(s_1,s_2)\right|ds_1ds_2.
		\end{aligned}
	\end{equation*}
	From \eqref{bounded_outputs_for_Gbnd}, we have that $|\phi_i(\mathbf{u}_{k},\Xi_{k})| = |v_{i,k}|\leq v_i^*$ for all $(\mathbf{u}_k,\Xi_k)\in\Omega\subseteq \mathbb{R}^m\times\mathbb{R}^n$ and, hence,
	\begin{equation*}
		\norm{\zeta}_1 \leq v_i^*\sum\limits_{j=1}^r\int_{\Omega}\left|{\psi}_j(s_1,s_2)\right|ds_1ds_2,
	\end{equation*}
	which results in
	\begin{equation*}
		\norm*{g_i^\top}_\infty \leq v_i^* \norm{\Gamma^{-1}}_1 \sum\limits_{j=1}^r\int_{\Omega}\left|{\psi}_j(s_1,s_2)\right|ds_1ds_2.
	\end{equation*}
	as in \eqref{G_bnd_a}.
\end{proof}
\begin{remark}
	Invertibility of the matrix $\Gamma$ in Lemma \ref{Lemma_G} is guaranteed if the basis functions are orthogonal in $\Omega$.
\end{remark}
\begin{remark}\label{remark_G}
	Since $\norm*{\mathcal{G}}_\infty = \max\limits_{i}\norm*{g_i^\top}_\infty = \max_i \norm*{g_i}_1$, then
	\begin{equation*}
		\norm*{\mathcal{G}}_\infty \leq v^* \norm*{\Gamma^{-1}}_1 \sum\limits_{j=1}^r\int_{\Omega}\left|{\psi}_j(s_1,s_2)\right|ds_1ds_2,
	\end{equation*}
	where $v^*\coloneqq\max\limits_i v_i^*$. Following similar arguments to Lemma \ref{Lemma_G}, one can obtain an upper bound on $\norm*{\mathcal{G}^\dagger}_\infty$, e.g., by using $\left< \mathcal{G}^\dagger\Phi(s_1,s_2) \hspace{-0.5mm}-\hspace{-0.5mm} {\Psi}(s_1,s_2) , \mathcal{G}^\dagger\Phi(s_1,s_2) \hspace{-0.5mm}-\hspace{-0.5mm} {\Psi}(s_1,s_2) \right>$ as the objective function of \eqref{def_of_G_mat}. Such a bound is required in the data-based nonlinear predictive control scheme in Section \ref{robust_nmpc_sec}.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Kernel approximation}
We conclude this section by illustrating how one can use kernel approximation methods from machine learning \cite{Hofmann08} to obtain an approximate solution to the data-driven simulation and output matching problems similar to Theorems \ref{MIMO_inexact_sim_thm} and \ref{MIMO_inexact_om_thm}, albeit without any guaranteed error bounds as in \eqref{err_sim} and \eqref{err_om}, respectively (cf. \cite{Berberich20, AlsaltiBerLopAll2021}).
%We conclude this section by showing a \emph{heuristic} method to solve the simulation and output-matching problems. In particular, one can use kernel approximation methods from machine learning \cite{Hofmann08} to obtain an approximate solution to the two problems similar to Theorems \ref{MIMO_inexact_sim_thm} and \ref{MIMO_inexact_om_thm}, albeit without any guaranteed error bounds as in \eqref{err_sim} and \eqref{err_om}, respectively (cf. \cite{Berberich20, AlsaltiBerLopAll2021}).
To apply such techniques, notice that the minimization problems in \eqref{alpha*} and \eqref{alpha*2} depend only on the inner product of the basis functions and not explicitly on the individual functions $\psi_i$ themselves. Therefore, one can \emph{implicitly} choose an infinite number of basis functions and approximate their inner product by, e.g., multi-variate Gaussian kernels of the following form
 \begin{gather}
		\hat{\Psi}_k(\mathbf{u},\Xi)^\top \hat{\Psi}_\ell(\mathbf{u},\Xi)=\exp\left(-\frac{1}{2\sigma^2}\norm*{\small\begin{bmatrix}\mathbf{u}_k\\\Xi_{k}\end{bmatrix}\hspace{-1mm}-\hspace{-1mm}\begin{bmatrix}\mathbf{u}_\ell\\\Xi_\ell\end{bmatrix}}_2^2\right)\hspace{-1mm}.
	\label{kernels}
\end{gather}
\indent However, (implicitly) using an infinite number of basis functions requires an infinitely long input-output sequence (since rank$(\hat{\Psi}(\mathbf{u},\Xi)+\hat{E}(\mathbf{u},\Xi))=r(L+n)$ is required in Theorems \ref{MIMO_sim_thm} and \ref{MIMO_om_thm}, respectively), which is not applicable in practice. Instead one can in general only approximate a subset of the input-output trajectory space. 
An interesting research problem is to find similar bounds to \eqref{err_sim} and \eqref{err_om} when using kernels such as the ones shown in \eqref{kernels} along with constructive guidelines on how to tune the corresponding hyperparameters.
